Fast MCMC sampling algorithms on polytopes

We propose and analyze two new MCMC sampling algorithms, the Vaidya walk and the John walk, for generating samples from the uniform distribution over a polytope. Both random walks are sampling algorithms derived from interior point methods. The former is based on volumetric-logarithmic barrier introduced by Vaidya whereas the latter uses John's ellipsoids. We show that the Vaidya walk mixes in significantly fewer steps than the logarithmic-barrier based Dikin walk studied in past work. For a polytope in $\mathbb{R}^d$ defined by $n >d$ linear constraints, we show that the mixing time from a warm start is bounded as $\mathcal{O}(n^{0.5}d^{1.5})$, compared to the $\mathcal{O}(nd)$ mixing time bound for the Dikin walk. The cost of each step of the Vaidya walk is of the same order as the Dikin walk, and at most twice as large in terms of constant pre-factors. For the John walk, we prove an $\mathcal{O}(d^{2.5}\cdot\log^4(n/d))$ bound on its mixing time and conjecture that an improved variant of it could achieve a mixing time of $\mathcal{O}(d^2\cdot\text{polylog}(n/d))$. Additionally, we propose variants of the Vaidya and John walks that mix in polynomial time from a deterministic starting point. The speed-up of the Vaidya walk over the Dikin walk are illustrated in numerical examples.

==> JohnWalkProofNew.tex <==
%!TEX root = PolytopeWalksUnifiedVersion_jmlr_submit.tex

\section{Analysis of the John walk}
\label{sec:proof_john_walk}

We recap the key ideas of the John walk for convenience.
We have designed a new proposal distribution by making use of an \emph{optimal set of weights}
to define the new covariance structure for the Gaussian proposals,
where optimality is defined with respect to the convex program defined
below~
\eqref{eq:john_convex_john_weights}.
The optimality condition is closely related to the problem of finding the largest ellipsoid at
any interior point of the polytope, such that the ellipsoid is contained within the polytope.
This problem of finding the largest ellipsoid was first studied by~\cite{joh48} who showed that each convex body in $\realdim$ contains a unique ellipsoid of maximal volume.
More recently,~\cite{lee2014path} make use of approximate John Ellipsoids to improve
the convergence rate of interior point methods for linear programming.
We refer the readers to their paper for more discussion about the use of John Ellipsoids
for optimization problems.
In this work, we make use of these ellipsoids for designing sampling algorithms with better theoretical
bounds on the mixing times.

The vector $\johnweights_{x} = \parenth{\johnweights_{x, 1}, \ldots, \johnweights_{x, \obs}}\tp$ defined in the John walk's inverse covariance matrix~\eqref{eq:john_covariance} is
computed by solving the following optimization problem:
\begin{align}
  \johnweights_x = \arg\min_{\weights \in \real^\obs} c_x\parenth{\weights} := \sum_{i=1}^\obs \weights_i - \frac{1}{\johnalpha} \log \det \parenth{A\tp \slackmatrix_x^{-1} \weightmatrix^{\johnalpha} \slackmatrix_x^{-1} A} - \johnbeta \sum_{i=1}^\obs \log \weights_i,
  \label{eq:john_convex_john_weights}
\end{align}
where the parameters $\johnalpha, \johnbeta$ are given by
\begin{align*}
  \johnalpha = 1 - \frac{1}{\log_2 \parenth{2\obs/\dims}}
   \quad\text{ and } \quad
   \johnbeta = \frac{\dims}{2\obs},
\end{align*}
and $\weightmatrix$ denotes an $\obs \times \obs$ diagonal matrix with $\weightmatrix_{ii} = \weights_i$ for each $i \in [\obs]$.
In particular, for our proposal the inverse covariance matrix is proportional to $\john_x$, where
\begin{align}
  \john_x =\sum_{i=1}^\obs \johnweights_{x, i}\frac{a_i a_i\tp} {(b_i -a_i\tp x)^2}.
  \label{eq:john_define_Jx}
\end{align}
where $\johnkappa \defn \johnkappa_{\obs, \dims} = \log_2(2\obs/\dims) = (1-\johnalpha)^{-1}$.

Recall that for John walk with parameter $\frac{r}{\dims^{3/4} \johnkappa^2}$, the proposals at state $x$ are
drawn from the multivariate Gaussian distribution given by $\NORMAL\parenth{x, \frac{r^2}{\dims^{3/2} \johnkappa^4} \john_x^{-1}}$,
which we denote by $\proposal_x^\tagjohn$.
In particular, the proposal density at point $x \in \intP$ is given by
\begin{align}
  \label{eq:john_proposal_density}
  \density_x(z)
  := \density(x, z)
  = \sqrt{\det{\john_x}} \parenth{\frac{\johnkappa^4 \dims^{3/2}}{2\pi r^2}}^{\dims/2} \exp\parenth{-\frac{\johnkappa^4 \dims^{3/2}}{2r^2} \ (z-x)\tp \john_x (z-x) }.
\end{align}
Here we restate our result for the mixing time of the John walk.
% start the theorem with Theorem 2. Theorem 1 is reserved for the Vaidya walk
\setcounter{theorem}{1}
\begin{theorem}
\label{thm:john_walk_1}
 Let $\initial$ be any distribution that is $M$-warm with respect to
$\stationary$ and let \mbox{$\obs < \exp(\sqrt{\dims})$}.  Then for any $\delta \in (0, 1]$, the John walk with parameter
  $\rparam_{\fulltagjohn} = \johnradiusconst$ satisfies
\begin{align*}
    \tvnorm{\plaintransition_{\fulltagjohn(\rparam)}^k(\initial) -\stationary} \leq
    \delta \qquad \text{ for all } k \geq C \; \dims^{2.5}\,
    \log_2^4\parenth{\frac{2\obs}{\dims}} \, \log\parenth{\frac{\sqrt{M}}{\delta}}.
  \end{align*}
\end{theorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Auxiliary results}
We begin by proving basic properties of the weights~$\johnweights_x$ which are used throughout the paper. For $x \in \intP, w \in \real^\obs_{++}$, define the projection matrix $\johnprojmatrix_{x, w}$ as follows
\begin{align}
  \johnprojmatrix_{x, w} = \weightmatrix^{\alpha/2} A_x (A_x^\top \weightmatrix^\alpha A_x)^{-1} A_x^\top \weightmatrix^{\alpha/2},
  \label{eq:john_projection_matrix}
\end{align}
where $A_x = \slackmatrix_x^{-1} A$ and $\weightmatrix$ is the $\obs \times \obs$ diagonal matrix with $i$-th diagonal entry given by $\weights_i$.
Also, let
\begin{align}
\levjohn_{x, i} \defn \parenth{\johnprojmatrix_{x, \johnweights_x}}_{ii} \quad \text{for } x \in \intP \text{ and } i \in [\obs].
\label{eq:john_first_Leverage_definition}
\end{align}
Define the \emph{John slack sensitivity} $\johnlocalslack_x^\tagjohn$ as
  \begin{align}
    \johnlocalslack_{x} \defn \johnlocalslack_x^\tagjohn \defn \parenth{\frac{a_1\tp \john_x^{-1} a_1}{\slack_{x, 1}^2}, \ldots, \frac{a_\obs\tp \john_x^{-1} a_\obs}{\slack_{x, \obs}^2}}\tp \quad \text{for all } x \in \intP.
    \label{eq:john_john_theta_defn}
  \end{align}
Further, for any $x \in \intP$,  define the \emph{John local norm at $x$} as
\begin{align}
  \label{eq:john_def_john_local_norm}
  \vecnorm{\cdot}{\john_x}: v \mapsto \vecnorm{\john_x^{1/2}v}{2} =
  \sqrt{\sum_{i=1}^\obs \johnweights_{x, i} \frac{(a_i\tp
      v)^2}{\slack_{x, i}^2}}.
\end{align}
We now collect some basic properties of the weights~$\johnweights_x$ and the local sensitivity~$\johnlocalslack_x$ and restate parts of Lemma~\ref{lemma:first_bounds} for clarity here.
\begin{lemma}
  \label{lemma:john_first_bounds}
  For any $x \in \intP$, the following properties are true:
  \begin{enumerate}[label=(\alph*)]
  \item (Implicit weight formula) \label{item:john_weight_equality} $\johnweights_{x, i} = \levjohn_{x, i} + \johnbeta$ for all $i \in [\obs]$,
  \item (Uniformity)\label{item:john_sigma_bound}
  $\johnweights_{x, i} \in [\johnbeta, 1+\johnbeta]$  for
      all $i \in [\obs]$,
  \item (Total size)\label{item:john_weight_sum}
  $\sum_{i=1}^\obs \johnweights_{x, i} = 3\dims/2$, and
  \item (Slack sensitivity)\label{item:john_theta_bound} $\johnlocalslack_{x, i} \in \brackets{0, 4}$ for
  all $i \in [\obs]$.
  \end{enumerate}
\end{lemma}
\noindent Lemma~\ref{lemma:john_first_bounds} follows from Lemmas~14 and 15 by~\cite{lee2014path} and thereby we omit its proof.


Next, we state a key lemma that is crucial for proving the convergence rate of John walk.
In this lemma, we provide bounds on difference in total variation norm between the proposal distributions of two nearby points.
\begin{lemma}
  \label{lemma:john_walk_close_kernel}
  \begin{subequations}
    There exists a continuous non-decreasing function $\johnradiusbound: [0, 1/30] \rightarrow \real_+$ with $\johnradiusbound(\johnepsilonconst) \geq \johnradiusconst$, such that for any
    $\epsilon \in (0, \johnepsilonconst]$, the John walk with $r \in [0, \johnradiusbound(\epsilon)]$ satisfies
    \begin{align}
      \tvnorm{\proposal^\tagjohn_x-\proposal^\tagjohn_y} &\leq
      \epsilon, \quad \mbox{for all $x, y \in \intP$ such that
        $\vecnorm{x-y}{\john_x} \leq \displaystyle\frac{\epsilon
          r}{2\johnkappa^2\dims^{3/4}}$ } ,\quad \text{and}
      %
      \label{eq:john_john_delta_p}\\
      \tvnorm{\plaintransition_{\fulltagjohn(\rparam)}(\diracdelta_x)-\proposal^\tagjohn_x} &\leq
      5\epsilon, \, \,\, \mbox{for all $x \in \intP$.}
      \label{eq:john_john_delta_q_p}
    \end{align}
  \end{subequations}
\end{lemma}
\noindent See Section~\ref{ssub:proof_of_lemma_lemma:john_walk_close_kernel} for its proof.

With these lemmas in hand, we are now ready to prove Theorem~\ref{thm:john_walk_1}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proof of Theorem~\ref{thm:john_walk_1}}
\label{sub:proof_of_theorem_thm:john_walk}
The proof is similar to the proof of Theorem~1, and relies on the Lov{\'a}sz's Lemma.
Here onwards, we use the following simplified notation
\begin{align*}
  \transition_x = \plaintransition_{\fulltagjohn(\rparam)}(\diracdelta_x), \proposal_x = \proposal_x^\tagjohn \text{ and }\vecnorm{\cdot}{x} = \vecnorm{\cdot}{\john_x}.
\end{align*}
In order to invoke Lov{\'a}sz's Lemma, we need to show that for any two points $x, y \in \intP$ with small cross-ratio $d_\Pspace(x, y)$, the TV-distance $\tvnorm{\transition_x-\transition_y}$ is also small.

We proceed with the proof in two steps: (A) first, we relate the cross-ratio $d_\Pspace(x, y)$ to the John local norm of $x-y$ at $x$, and (B) we then use Lemma~\ref{lemma:john_walk_close_kernel} to show that if $x, y \in \intP$ are close in the John local-norm, then the transition kernels $\transition_x$ and $\transition_y$ are close in TV-distance.

\paragraph{Step~(A):}
\label{par:step_a_john}
We claim that for all $x, y \in \intP$, the cross-ratio can be lower
bounded as
\begin{align}
  d_\Pspace(x, y) \geq \frac{1}{\sqrt{3\dims/2}} \vecnorm{x-y}{x}.
  \label{eq:john_hilbert_to_local_john}
\end{align}
From the arguments in the proof of Theorem~1 (proof for the Vaidya Walk), we have
\begin{align}
d_\Pspace(x, y) \geq \max_{i \in [\obs]} \left\vert\frac{a_i\tp (x - y)}{\slack_{x, i}}
  \right\vert.
  \label{eq:john_relate_cross_ratio_john}
\end{align}
Using the fact that maximum of a set of non-negative numbers is greater than the
weighted mean of the numbers and Lemma~\ref{lemma:john_first_bounds}, we find that
% Combining this fact with properties
% \ref{item:sigma_bound} and \ref{item:sigma_sum} from
% Lemma~\ref{lemma:first_bounds}, we find that
\begin{align*}
  d_\Pspace(x, y) \geq \sqrt{ \frac{1}{\sum_{i=1}^\obs
    \johnweights_{x, i}} \sum_{i=1}^\obs
  \johnweights_{x, i} \frac{(a_i \tp (x-y))^2}
  {\slack_{x, i}^2}} = \frac{\vecnorm{x-y}{x}}{\sqrt{3\dims/2}},
\end{align*}
thereby proving the claim~\eqref{eq:john_hilbert_to_local_john}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\paragraph{Step~(B):}
\label{par:step_b_john}
By the triangle inequality, we have
\begin{align*}
  \tvnorm{\transition_x - \transition_y} \leq
  \tvnorm{\transition_x-\proposal_x} + \tvnorm{\proposal_x-\proposal_y}
  + \tvnorm{\proposal_y - \transition_y}.
\end{align*}
Using Lemma~\ref{lemma:john_walk_close_kernel}, we obtain that
\begin{align*}
\tvnorm{\transition_x - \transition_y} & \leq 11 \epsilon, \quad
\mbox{$\forall x, y \in \intP$ such that $ \vecnorm{x-y}{x} \leq
  \displaystyle \frac{\epsilon
          r}{2\johnkappa^2\dims^{3/4}} $}.
\end{align*}
Consequently, the John walk satisfies the assumptions of
Lov{\'a}sz's Lemma with
\begin{align*}
  \Delta \defn \frac{1}{\sqrt{3\dims/2}} \cdot \frac{\epsilon
          r}{2\johnkappa^2\dims^{3/4}} \quad \mbox{and} \quad \rho \defn 1 - 11\epsilon.
\end{align*}
Plugging in $\epsilon = 1/30$, $r = 10^{-5}$, we obtain the claimed upper bound of $\order{\johnkappa^4 \dims^{5/2}}$
on the mixing time of the random walk.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proof of Lemma~\ref{lemma:john_walk_close_kernel}}
\label{ssub:proof_of_lemma_lemma:john_walk_close_kernel}
We prove the lemma for the following function,
\begin{align*}
  \johnradiusbound(\epsilon) &= \min \braces{\frac{1}{25\sqrt{1+\sqrt{2}\log(4/\epsilon)}}, \frac{\epsilon}{\parenth{2\sqrt{32}\tailconstjohn_{1, \epsilon}}}, \sqrt{\frac{\epsilon}{386\sqrt{24}\tailconstjohn_{2, \epsilon}}}, \frac{\epsilon}{5\sqrt{60} \tailconstjohn_{3, \epsilon}}, \right. \\
  &\left. \sqrt{\frac{\epsilon}{8\sqrt{1680} \tailconstjohn_{4, \epsilon}}}, \sqrt{\frac{\epsilon}{40\parenth{\tailconstjohn_{2, \epsilon}\tailconstjohn_{6, \epsilon} \sqrt{24}\sqrt{15120}}^{1/2}}}, \sqrt{\frac{\epsilon}{204800\tailconstjohn_{2, \epsilon}\sqrt{24}\log(32/\epsilon)}}}.
\end{align*}
where $\tailconstjohn_{1, \epsilon} = \log(2/\epsilon)$and $\tailconstjohn_{\degree, \epsilon} = \parenth{2e/\degree \cdot \log\parenth{16/\epsilon}}^{\degree/2}$ for \mbox{$\degree = 2,
     3, 4$ and $6$}. A numerical calculation shows that $\johnradiusbound(\johnepsilonconst) \geq \johnradiusconst$.

% \yccomment{Remark: these conditions are collected from conditions~\eqref{eq:john_whp_slackness_r_condition}~\eqref{eq:john_gradient_log_det_tail_r_condition}~\eqref{eq:john_hessian_log_det_tail_r_condition}~\eqref{eq:john_gradient_local_norm_tail_r_condition} and~\eqref{eq:john_hessian_local_norm_tail_r_condition}.}


We now prove the two parts~\eqref{eq:john_john_delta_p}~\eqref{eq:john_john_delta_q_p} of the Lemma separately.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Proof of claim~(\ref{eq:john_john_delta_p})}
\label{sssub:proof_of_claim_eq:john_john_delta_p}

Applying Pinsker's inequality, and plugging in the closed formed expression for the KL divergence between two Gaussian distributions we find that
\begin{align}
  \label{eq:john_final_KL_expression_john}
  \tvnorm{\proposal_x-\proposal_y}^2 \leq 2 \kldiv{\proposal_y}{\proposal_x}
  & = \trace(\john_x^{-1/2} \john_y \john_x^{-1/2})
    \!-\!\dims\!-\!\log\det(\john_x^{-1/2}
    \john_y \john_x^{-1/2}) + \frac{\johnkappa^4\dims^{3/2}}{r^2} \vecnorm{x\!-\!y}{x}^2 \notag \\
  & = \sum_{i=1}^\dims \parenth{\lambda_i - 1 + \log\frac{1}{\lambda_i}}
    + \frac{\johnkappa^4\dims^{3/2}}{r^2} \vecnorm{x-y}{x}^2,
\end{align}
where $\lambda_1, \ldots, \lambda_\dims >0$ denote the eigenvalues of the matrix $\john_x^{-1/2} \john_y \john_x^{-1/2}$.
% , and we have used the facts that $\det(\john_x^{-1/2} \john_y \john_x^{-1/2}) = \prod_{i=1}^\dims \lambda_i$
% and $\trace({\john_x^{-1/2} \john_y \john_x^{-1/2}}) = \sum_{i=1}^\dims \lambda_i$.
To bound the expression~\eqref{eq:john_final_KL_expression_john}, we make use of the following lemma:

\begin{lemma}
  \label{lemma:john_close_hessian_eigenvalues}
  For any scalar $t \in [0, 1/64]$ and  pair of points $x, y \in
  \intP$ such that \mbox{$\vecnorm{x-y}{x} \leq t / \johnkappa^2$,}
  we have
  \begin{align*}
    \parenth{1-48t+4t^2} \Ind_\dims
    \preceq \john_x^{-1/2} \john_y \john_x^{-1/2} \preceq \parenth{1+48t+4t^2},
  \end{align*}
  where $\preceq$ denotes ordering in the PSD cone and $\Ind_\dims$ denotes the $\dims$-dimensional identity matrix.
\end{lemma}
\noindent See Section~\ref{sec:proof_of_lemma_lemma:john_close_hessian_eigenvalues}
 for the proof of this lemma.

For $\epsilon \in (0, \johnepsilonconst]$ and $r = \johnradiusconst$, we have $t = \epsilon r /(2\dims^{3/4}) \leq 1/64$, whence the eigenvalues $\{\lambda_i, i \in [\dims]\}$ can be sandwiched as
\begin{align}
  \label{eq:john_lambda_bounds_john}
  1 - \frac{24 \epsilon r}{\dims^{3/4}} + \frac{\epsilon^2r^2}{\dims^{3/2}}
  \leq \lambda_i
  \leq  1 + \frac{24 \epsilon r}{\dims^{3/4}} + \frac{\epsilon^2r^2}{\dims^{3/2}}
  \quad \mbox{for all $i \in \dims$}.
\end{align}
We are now ready to bound the TV distance between $\proposal_x$ and $\proposal_y$.
Using the bound~\eqref{eq:john_final_KL_expression_john} and the inequality $\log \omega \leq \omega - 1$, valid for $ \omega > 0$, we obtain
\begin{align*}
\tvnorm{\proposal_x-\proposal_y}^2 \leq \sum_{i=1}^\dims
\parenth{\lambda_i - 2 + \frac{1}{\lambda_i}} + \frac{\johnkappa^4\dims^{3/2}}{r^2} \vecnorm{x-y}{x}^2.
\end{align*}
Using the assumption that $\vecnorm{x-y}{x}\leq {\epsilon r}/\parenth{2\johnkappa^2\dims^{3/4}}$, and plugging in the bounds~\eqref{eq:john_lambda_bounds_john} for the eigenvalues $\{\lambda_i, i \in [\dims]\}$, we find that
\begin{align*}
  \sum_{i=1}^\dims \parenth{\lambda_i - 2 + \frac{1}{\lambda_i}}
  + \frac{\johnkappa^4\dims^{3/2}}{r^2} \vecnorm{x-y}{x}^2 \leq \frac{2000
    \epsilon^2 r^2}{\sqrt{\dims}} + \frac{\epsilon^2}{4}.
\end{align*}
In asserting this inequality, we have used the facts that
\begin{align*}
  \frac{1}{1 - 24\omega + \omega^2} \leq 1 + 24 \omega + 1000 \omega^2,
  \quad \text{and}\quad \frac{1}{1 + 24\omega + \omega^2} \leq 1 -
  24\omega + 1000 \omega^2 \quad \mbox{for all $\omega \in \brackets{0,
      \frac{1}{100}}$}.
\end{align*}
Note that for any $r \in [0, 1/100]$, we have that $2000 r^2/\sqrt{\dims} \leq 1/2$.
Putting the pieces together yields $\tvnorm{\proposal_x-\proposal_y} \leq \epsilon$, as claimed.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Proof of claim~(\ref{eq:john_john_delta_q_p})}
\label{sssub:proof_of_claim_eq:john_john_delta_q_p}
We have
\begin{align}
  \label{eq:john_bound_on_jumping_out}
  \tvnorm{\proposal_x - \transition_x}
  &\leq \underbrace{\frac{3}{2} \proposal_x(\Pspace^c)}_{= : \; S_1} +
  \underbrace{1-\Exs_{z \sim \proposal_x} \brackets{\min\braces{1,
       \frac{\density_z(x)}{\density_x(z)}}}}_{= : \; S_2},
\end{align}
where $\Pspace^c$ denotes the complement of $\Pspace$.
% Consequently, it suffices to show that both $S_1$ and $S_2$ are small, where the probability is taken over the randomness in the proposal $z$.
We now show that $S_1 \leq \epsilon$ and $S_2 \leq 4\epsilon$, from which the claim follows.  \\


\noindent \textbf{Bounding the term $S_1$:}
% Since $z$ is multivariate Gaussian with mean $x$ and covariance
% $\frac{r^2}{\johnkappa^2\dims^{3/2}} \john_x^{-1}$,
Note that for $z \sim \NORMAL(x, \frac{r^2}{\johnkappa^2\dims^{3/2}} \john_x^{-1})$, we can write
\begin{align}
  \label{eq:john_z_x_relation}
  z \stackrel{d}{=} x + \frac{r}{\johnkappa\dims^{3/4}}
  \john_x^{-{1}/{2}} \rvg,
\end{align}
where $\rvg \sim \NORMAL\parenth{0, \Ind_\dims}$ and $\stackrel{d}{=}$
denotes equality in distribution.
Using equation~\eqref{eq:john_z_x_relation} and definition~\eqref{eq:john_john_theta_defn} of $\localslack_{x, i}$, we obtain the bound
\begin{align}
  \label{eq:john_bound_on_deviation}
  \frac{\parenth{a_i \tp \parenth{z-x}}^2 }{\slack_{x, i}^2} & =
  \frac{r^2}{\johnkappa^2\dims^{3/2}}
  \brackets{\frac{a_i \tp \john_x^{-{1}/{2}} \rvg }{\slack_{x,
       i}}}^2 \stackrel{(i)}{\leq} \frac{r^2}{\johnkappa^2\dims^{3/2}} \localslack_{x, i}
  \vecnorm{\rvg}{2}^2 \stackrel{(ii)}{\leq} \frac{4r^2}{\dims}
  \vecnorm{\rvg}{2}^2,
\end{align}
where step $(i)$ follows from Cauchy-Schwarz inequality, and step $(ii)$ from part~\ref{item:john_theta_bound} of Lemma~\ref{lemma:john_first_bounds}.
Define the events
\begin{align*}
  \mathcal{E} \defn \braces{\frac{r^2}{\dims} \vecnorm{\rvg}{2}^2 < \frac{1}{4}}
  \quad \text{and} \quad
  \mathcal{E}'\defn \braces{z \in \intP}.
\end{align*}
Inequality~\eqref{eq:john_bound_on_deviation} implies that $\mathcal{E}
\subseteq \mathcal{E}'$ and hence $\Prob\brackets{\mathcal{E}'} \geq
\Prob\brackets{\mathcal{E}}$.  Using a standard Gaussian tail bound
and noting that $r \leq \frac{1/2}{1 + \sqrt{2/\dims \log
    (2/\epsilon)}}$, we obtain $ \Prob\brackets{\mathcal{E}} \geq
1-\epsilon/2$ and whence $ \Prob\brackets{\mathcal{E}'} \geq
1-\epsilon/2$.  Thus, we have shown that $\Prob\brackets{z
  \notin \Pspace} \leq \epsilon/2$ which implies that $S_1 \leq
\epsilon$.  \\

\noindent \textbf{Bounding the term $S_2$:}
By Markov's inequality, we have
\begin{align}
  \label{eq:john_markov_inequality}
  \Exs_{z \sim \proposal_x} \brackets{\min\braces{1,
            \frac{\density_z(x)}{\density_x(z)}}} \geq \alpha
        \Prob\brackets{\density_z(x) \geq \alpha \density_x(z)} \quad
        \mbox{for all $\alpha \in (0,
          1]$}.
\end{align}
By definition~\eqref{eq:john_proposal_density} of $\density_x$, we obtain
\begin{align*}
\frac{\density_z(x)}{\density_x(z)} = \exp
\parenth{-\frac{\dims^{3/2}\johnkappa^4}{2r^2} \parenth{\vecnorm{z-x}{z}^2-
    \vecnorm{z-x}{x}^2 }+ \frac{1}{2} \parenth{\log \det \john_z -
    \log \det \john_x}}.
\end{align*}
The following lemma provides us with useful bounds on the two terms in
this expression, valid for any $x \in \intP$.
\begin{lemma}
 \label{lemma:john_change_in_log_det_and_local_norm}
  For any $\epsilon \in (0, \frac{1}{4}]$ and $r \in (0, \johnradiusbound(\epsilon)]$,
     we have
  \begin{subequations}
    \begin{align}
      \label{eq:john_whp_log_det_filter}
      \Prob_{z\sim \proposal_x}\brackets{\frac{1}{2}\log\det \john_z
       - \frac{1}{2}\log\det \john_x \geq -\epsilon } &\geq 1 -
      \epsilon,
      \quad  \text{and}
      \\
      %
      \label{eq:john_whp_local_norm}
      \Prob_{z\sim \proposal_x}\brackets{\vecnorm{z - x}{z}^2 - \vecnorm{z -
      x}{x}^2 \leq 2 \epsilon \frac{r^2}{\johnkappa^4 \dims^{3/2}}} &\geq
      1 - \epsilon.
    \end{align}
   \end{subequations}
\end{lemma}
\noindent We provide the  of this lemma in Section~\ref{sec:proof_of_lemma_lemma:john_change_in_log_det_and_local_norm}.

Using Lemma~\ref{lemma:john_change_in_log_det_and_local_norm}, we now
 complete the proof of the Theorem~\ref{thm:john_walk_1}.  For $r \leq \johnradiusbound(\epsilon)$, we obtain
\begin{align*}
  \frac{\density_z(x)}{\density_x(z)} & \geq \exp\parenth{-2\epsilon}
  \geq 1- 2 \epsilon
\end{align*}
 with probability at least $1-2\epsilon$.
 Substituting $\alpha = 1- 2 \epsilon$ in inequality~\eqref{eq:john_markov_inequality} yields that $S_2 \leq 4 \epsilon$, as claimed.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Technical Lemmas for the John walk} % (fold)
\label{sec:technical_lemmas}

We begin by summarizing a few key properties of various terms involved
in our analysis.

% We begin with some notation and intermediate expansions of terms that are useful for the proofs later on.
\begin{subequations}
Let $\johnlevmatrix_{x, w}$ be an $\obs \times \obs$ diagonal matrix defined as
\begin{align}
    \johnlevmatrix_{x, w} &= \diag\parenth{\levjohn_{x, w, i}, \ldots, \levjohn_{x, w, \obs}} \text{ where } \levjohn_{x, \johnweights_x, w, i} = (\johnprojmatrix_{x, w})_{ii}, i\in[\obs].
    \label{eq:john_john_Leverage_definition}
% \end{align}
% Let $\johnlevmatrix_{x, w}$ be an $\obs \times \obs$ diagonal matrix defined as
% \begin{align}
%     \johnlevmatrix_{x, w} &= \diag\parenth{\levjohn_{x, w, i}, \ldots, \levjohn_{x, w, \obs}} \text{ where } \levjohn_{x, w, i} =  (\johnprojmatrix_{x, w})_{ii}, i\in[\obs].
%     \label{eq:john_Leverage_definition}
\end{align}Let $\johnprojmatrix_{x, w}^{(2)}$ denote the hadamard product of $\johnprojmatrix_{x, w}$ with itself.
Further define
\begin{align}
    \johnlaplacian_{x, w} := \johnlevmatrix_{x, w} - \johnprojmatrix_{x, w}^{(2)}.
    \label{eq:john_lambda}
\end{align}
\end{subequations}
\begin{subequations}
\cite{lee2014path} proved that the weight vector $\johnweights_x$ is the unique solution of the following fixed point equation:
\begin{align}
    \weights_i = \levjohn_{x, \weights, i} + \johnbeta, i \in [\obs].
    \label{eq:john_fixed_point_equation_john_weights}
\end{align}
To simplify notation, we use the following shorthands:
\begin{align}
    \levjohn_x = \levjohn_{x, \johnweights_x}, \quad \johnprojmatrix_x = \johnprojmatrix_{x, \johnweights_x}, \quad \johnprojmatrix_x^{(2)} = \johnprojmatrix_{x, \johnweights_x}^{(2)}, \quad \johnlevmatrix_x = \johnlevmatrix_{x, \johnweights_x}, \quad \johnlaplacian_x = \johnlaplacian_{x, \johnweights_x}.
\end{align}
Thus, we have the following relation:
\begin{align}
    \johnweights_x = \levjohn_{x, \johnweights_x} + \johnbeta \mathbf{1} = \levjohn_x + \johnbeta \mathbf{1}.
    \label{eq:john_normal_equation}
\end{align}
\end{subequations}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Deterministic expressions and bounds} % (fold)
\label{sub:deterministic_bounds}

We now collect some properties of various terms defined above.
%
\begin{lemma}
  \label{ppt:john_all_properties}
  For any $x \in \intP$, the following properties hold:
  \begin{enumerate}[label=(\alph*)]
    \item\label{item:john_sigma_properties} $\levjohn_{x, i} =
    \sum_{j=1}^\obs \levjohn^2_{x, i, j} = \sum_{j, k=1}^\obs
    \levjohn_{x, i, j} \levjohn_{x, j, k} \levjohn_{x, k,
      i}$ for each $i \in [\obs]$,
    %
    \item\label{item:john_Sigma_dominates_P} $\johnlevmatrix_x
    \succeq \johnprojmatrix_x^{(2)}$,
    %
    \item\label{item:john_theta_sum} $\sum_{i=1}^\obs \johnweights_{x, i} \johnlocalslack_{x, i}
    = \dims$,
    %
    \item\label{item:john_theta_properties} $\johnlocalslack_{x, i} = \sum_{j=1}^\obs \johnweights_{x, i} \johnlocalslack_{x, i, j}^2$, for each $i \in
               [\obs]$,
    %
    \item\label{item:john_theta_square_sigma_sum_bound}
    $\johnlocalslack_x \tp \johnlevmatrix_x \johnlocalslack_x = \sum_{i=1}^\obs
    \johnlocalslack_{x, i}^2 \johnweights_{x, i}
    \leq 4 \dims$, and
    %
    \item \label{item:john_W_sandwich} $\displaystyle\johnbeta\,
    \hesslogbarr_x \preceq \john_x \preceq \parenth{1 + \johnbeta}
    \hesslogbarr_x$.
  \end{enumerate}
\end{lemma}
The proof is based on the ideas similar to Lemma 5 in the proof of the Vaidya walk and is thereby omitted.

The next lemma relates the change in \emph{slackness} $\slack_{x, i} = b_i-a_i\tp x$ to the John-local norm at $x$.
\begin{lemma}
  \label{lemma:john_closeness_of_slackness}
  For all $x, y \in \intP$, we have
  \begin{align*}
    \max_{i\in[\obs]}\abss{1 - \frac{\slack_{y,i}}{\slack_{x,i}}} \leq 2 \vecnorm{x - y}{x}.
  \end{align*}
\end{lemma}
\begin{proof}
  For any pair $x, y \in \intP$ and index $i \in [\obs]$, we have
  \begin{align*}
   \parenth{a_i \tp \parenth{x-y}}^2
   % = \parenth{(\john_x^{-\frac{1}{2}} a_i) \tp \john_x^{\frac{1}{2}}(x-y)}^2
   \stackrel{(i)}{\leq} \| \john_x^{-\frac{1}{2}} a_i\|^2_2 \; \|
   \john_x^{\frac{1}{2}} (x-y) \|^2_2
   % & = a_i^T \john_x^{-1} a_i \;  \vecnorm{x - y}{x}^2\\
   = \johnlocalslack_{x, i} \slack_{x, i}^2 \; \vecnorm{x -
     y}{x}^2
   \stackrel{(ii)}{\leq} 4 \slack_{x, i}^2
   \; \vecnorm{x - y}{x}^2,
  \end{align*}
  where step (i) follows from the Cauchy-Schwarz inequality, and step
  (ii) uses the bound $\johnlocalslack_{x, i}$ from
  Lemma~\ref{lemma:john_first_bounds}\ref{item:john_theta_bound}.  Noting the
  fact that $a_i\tp(x-y) = \slack_{y, i} - \slack_{x, i} $, the claim
  follows after simple algebra.
\end{proof}

We now state various expressions and bounds for the first and second order derivatives of the different terms.
To lighten notation, we introduce some shorthand notation.
For any $y \in \intP$ and $h \in \realdim$, define the following terms:
\begin{subequations}
  \begin{align}
    \projd_{y, i} &= \frac{a_i\tp h}{\slack_{y, i}}, \ i \in [\obs]
    &\projdmatrix_y &= \diag(\projd_{y, 1}, \ldots, \projd_{y, \obs}),
    \label{eq:john_def_D}\\
    \projf_{y, i} &= \frac{\nabla \johnweights_{y, i}\tp h}{\johnweights_{y, i}}, \ i \in [\obs]
    &\projfmatrix_y &= \diag(\projf_{y, 1}, \ldots, \projf_{y, \obs}),
    \label{eq:john_def_F}\\
    \projz_{y, i}& = \frac{1}{2} h\tp \nabla^2 \johnweights_{y, i} h / \johnweights_{y, i}, \ i \in [\obs]
    &\projzmatrix_y &= \diag(\projz_{y, 1}, \ldots, \projz_{y, \obs}),
    \label{eq:john_def_Z}\\
    \projzsub_y &\defn \parenth{\johnweightmatrix_y - \alpha \johnlaplacian_y}\begin{bmatrix} \projz_{y, 1} \\ \vdots \\ \projz_{y, \obs} \end{bmatrix}, \label{eq:john_def_rho}
  \end{align}
\end{subequations}
where for brevity in our notation we have omitted the dependence on $h$.
The choice of $h$ is specified as per the context.
Further, we define for each $x \in \intP$ and $i \in [\obs]$
\begin{align}
  \johnphi_{x,i} &\defn \displaystyle\frac{\johnweights_{x, i}}{\slack_{x, i}^2}, \quad
  &\text{and}& \quad &\logdetJ_x &\defn\frac{1}{2}\log \det
  \john_x,\\
  \hat{a}_{x, i} &\defn \frac{\john_x^{-1/2} a_{x, i}}{s_{x, i}^2}, \quad&\text{and}&\quad &\hat{b}_{x, i} &\defn\john_x^{-1/2}A_x\Lambda_x \parenth{G_x - \alpha \Lambda_x}^{-1} e_i.
  \label{eq:john_hat_a_hat_b}
\end{align}
Next, we state expressions for gradients of $\johnweights, \johnphi$ and
$\logdetJ$ and bounds for directional Hessian of $\levjohn$, $\johnphi$ and
$\logdetJ$ which are used in various Taylor series expansions and bounds in our proof.

\begin{lemma}[Calculus]
  \label{lemma:john_gradient_and_hessian_and_bounds}
  For any $y \in \intP$ and $h \in \real^\obs$, the following relations hold;
  \begin{enumerate}[label=(\alph*)]
    \item\label{item:gradient_g} Gradient of $\johnweights$:
    $(\projf_{y, 1}, \ldots, \projf_{y, \obs})\tp = 2 \parenth{\johnweightmatrix_y - \alpha \johnlaplacian_y}^{-1} \johnlaplacian_y A_y h$;
  %
    \item\label{item:hessian_g} Hessian of $\johnweights$:
    % \begin{align}
    %   \label{eq:john_weights_hessian_term_bound}
    %   \abss{\projzsub_{y, i}}
    %   \leq 7 \levjohn_{y, i} \projd_{y, i}^2 + 3 \levjohn_{y, i} \projf_{y, i}^2 + \sum_{j=1}^\obs \parenth{ 13\projd_{y, j}^2 + 6 \projf_{y, j}^2} \johnprojmatrix_{y, i, j}^2.
    % \end{align}
    \begin{align}
    \label{eq:john_l1_norm_on_weights_hessian}
      \vecnorm{\projzsub_y}{1}\leq 56 \johnkappa^2 \sum_{i=1}^\obs \johnweights_{y, i} \projd_{y, i}^2.
    \end{align}
%
    \item \label{item:gradient_log_det} Gradient of $\logdetJ$:
    $\nabla \logdetJ \tp h = \johnlocalslack_y\tp \johnweightmatrix_y \parenth{\Ind_\obs + \parenth{\johnweightmatrix_y - \alpha \johnlaplacian_y}^{-1}\johnlaplacian_y} A_y h$.

%
    % \item \label{item:hessian_log_det} Hessian of $\logdetJ$:
    % \begin{align*}
    %   \frac{1}{2} h \tp \hesslogdetJ_y h
    %   = \frac{1}{2}\brackets{\sum_{i=1}^\obs \johnweights_{y, i} \johnlocalslack_{y, i} (3\projd_{y, i}^2 + 2 \projd_{y, i}\projf_{y, i} + \projz_{y, i}) - \frac{1}{2} \sum_{i, j=1}^\obs \johnweights_{y, i} \johnweights_{y, j} \johnlocalslack_{y, i, j}^2 \parenth{2\projd_{y, i} + \projf_{y, i}} \parenth{2\projd_{y, j} + \projf_{y, j}}}.
    % \end{align*}
%
    \item\label{item:gradient_phi} Gradient of $\johnphi$: $\nabla \johnphi_{y, i}\tp h = \johnphi_{y, i} \parenth{2 \projd_{y, i} + \projf_{y, i}}$.
%
    % \item\label{item:hessian_phi} Hessian of $\johnphi$: $\frac{1}{2} h\tp \nabla^2 \johnphi_{y, i} h = \johnphi_{y, i} \parenth{2 \projd_{y, i} \projf_{y, i} + 3 \projd_{y, i}^2 + \projz_{y, i}}$.
%
    \item\label{item:john_hessian_log_det_bound} Bound on $\hesslogdetJ$:
    $\frac{1}{2} \abss{h\tp (\nabla^2 \logdetJ) h}
    \leq \frac{1}{2}\brackets{\sum_{i=1}^\obs \johnweights_{y, i}\, \johnlocalslack_{y, i} \brackets{ 9\, \projd_{y, i} ^2 + 4 \projf_{y, i}^2}   +  \abss{ \sum_{i=1}^\obs \johnweights_{y, i}\, \johnlocalslack_{y, i} \projz_{y, i}}}$
%
    \item \label{item:hessian_beta_bound} Bound on $\nabla^2\johnphi$:
    \begin{align*}
      \abss{\sum_{i=1}^\obs \projd_{y, i}^2 \slack_{y, i}^2 \frac{1}{2} h\tp \nabla^2 \johnphi_{y, i} h} \leq 3 \sum_{i=1}^\obs \johnweights_{y, i} \projd_{y, i}^4 + 2\abss{\sum_{i=1}^\obs \johnweights_{y,i} \projd_{y, i}^3 \projf_{y, i}} + \abss{\sum_{i=1}^\obs \johnweights_{y, i} \projd_{y, i}^2 \projz_{y, i}}.
    \end{align*}
  \end{enumerate}
\end{lemma}
The proof is provided in Section~\ref{sub:proof_of_lemma_lemma:john_gradient_and_hessian_and_bounds}.

Next, we state some results that would be useful to provide explicit bounds for various terms like $\projf_y, \projz_y$ and $\projzsub_y$ that appear in the statements of the previous lemma.
Note that the following results do not have a corresponding analog in our analysis of the Vaidya walk.
\begin{lemma}
  \label{lemma:f_to_d_l2}
  For any $c_1, c_2 \geq 0$, $y\in \intP$, we have
  \begin{align*}
    \parenth{c_1 \Ind_\obs + c_2 \johnlaplacian_y \parenth{\johnweightmatrix_y-\alpha\johnlaplacian_y}^{-1}} \johnweightmatrix_y \parenth{c_1 \Ind_\obs + c_2 \parenth{\johnweightmatrix_y-\alpha \johnlaplacian_y}^{-1} \johnlaplacian_y} \preceq \parenth{c_1 + c_2}^2 \johnkappa^2 \johnweightmatrix_y,
  \end{align*}
  where $\preceq$ denotes the ordering in the PSD cone.
\end{lemma}
\begin{lemma}
  \label{lemma:f_to_d_matrix}
    Let $\johnftdinvmatrix_{y}$ denote the $\obs \times \obs$ matrix $\parenth{\johnweightmatrix_y-\alpha\johnlaplacian_y}^{-1} \johnweightmatrix_y$, and let $\johnftdinvmatrix_{y, i, j}$ denote its $ij$-th entry.
    Then for each $i \in [\obs]$ and $y \in \intP$, we have
    \begin{subequations}
    \begin{align}
      \johnftdinvmatrix_{y, i, i} &\in [0, \johnkappa], \quad \text{ and, } \label{eq:john_mu_first_coordinate_bound}\\
      \sum_{j \neq i, j \in [\obs]} \frac{\johnftdinvmatrix_{y, i, j}^2}{\johnweights_{y, j}} &\leq \johnkappa^3.\label{eq:john_mu_sum_of_terms_bound}
    \end{align}
    \end{subequations}
\end{lemma}
\begin{corollary}
  \label{corollary:f_to_d_l1}
    Let $e_i \in \real^\obs$ denote the unit vector along $i$-th axis. Then for any $y\in \intP$, we have
    \begin{align}
    \label{eq:john_mu_1_bound}
      \vecnorm{\johnweightmatrix_y \parenth{\johnweightmatrix_y-\alpha\johnlaplacian_y}^{-1} e_i}{1} \leq 3 \sqrt{\dims} \johnkappa^{3/2}, \quad \text{ for all } i \in [\obs].
    \end{align}
    Consequently, we also have $\matsnorm{\parenth{\johnweightmatrix_y-\alpha\johnlaplacian_y}^{-1} \johnweightmatrix_y}{\infty} \leq 3 \sqrt{\dims} \johnkappa^{3/2}.$
\end{corollary}
See Section~\ref{sub:proof_of_lemma_lemma:f_to_d_l2}, \ref{sub:proof_of_lemma_lemma:f_to_d_matrix} and \ref{sub:proof_of_corollary_corollary:f_to_d_l1} for the proofs of Lemma~\ref{lemma:f_to_d_l2}, Lemma~\ref{lemma:f_to_d_matrix} and Corollary~\ref{corollary:f_to_d_l1} respectively.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Tail Bounds} % (fold)
\label{sub:tail_bounds}
We now collect lemmas that provide us with useful tail bounds.

We start with a result that shows that for a random variable $z \sim
\proposal_x$, the slackness $\slack_{z, i}$ is close to $\slack_{x,
  i}$ with high probability and consequently the weights $\johnweights_{z, i}$ are also close to $\johnweights_{x, i}$.
This result comes in handy for transferring the remainder terms in Taylor expansions to the reference point (around which the series is being expanded).

\begin{lemma}
  \label{lemma:john_whp_slackness}
  For any point $x \in \intP$ and $r \leq  \frac{1}{25 \cdot \sqrt{1+\sqrt2 \log(4/\epsilon)}}$, we have
  \begin{subequations}
    \begin{align}
      \label{eq:john_slack_whp}
      \Prob_{z \sim \proposal_x} \brackets{ \forall i \in [\obs],
        \forall v \in \overline{xz},\ {\frac{\slack_{x,
              i}}{\slack_{v, i}}} \in \brackets{0.99, 1.01}\text{ and }{\frac{\johnweights_{x, i}}{\johnweights_{v, i}}} \in \brackets{0.96, 1.04}}
              &\geq 1 - \epsilon/4
      \end{align}
  \end{subequations}
\end{lemma}
See Section~\ref{sub:proof_of_lemma_whp:slackness} for the proof of this lemma.

Next, we state high probability results for some Gaussian polynomials.
These results are useful to bound various polynomials of the form $\sum_{i=1}^\obs \johnweights_{x, i} \projd_{x, i}^k$, where $\projd_{x, i} = a_i\tp(z-x)/\slack_{x, i}$ and $z$ is drawn from the transition distribution for the John walk at point $x$.


\begin{lemma}[Gaussian moment bounds]
  \label{lemma:john_gaussian_moment_bounds}
  To simplify notations, all subscripts on $x$ are omitted in the following statements.
  For any $\epsilon \in (0, 1/30]$, define $\tailconstjohn_k \defn \tailconstjohn_{k, \epsilon} = \parenth{2e/k \cdot \log \parenth{16/\epsilon}}^{k/2}$, for $k=2,3,4\text{ and }6$, then we have
  \begin{subequations}
  \begin{align}
    \Prob\brackets{\sum_{i=1}^\obs \johnweights_i \parenth{\hat{a}_i\tp \rvg}^2 \leq \tailconstjohn_2 \sqrt{24}\dims} &\geq 1-\frac{\epsilon}{16},
    \label{eq:john_john_quadratic} \\
%
    \Prob\brackets{\sum_{i=1}^\obs \johnweights_i \parenth{\hat{a}_i\tp \rvg}^3 \leq \tailconstjohn_3 \sqrt{60}\dims^{1/2}} &\geq 1-\frac{\epsilon}{16},
    \label{eq:john_john_cubic} \\
%
    \Prob\brackets{\sum_{i=1}^\obs \johnweights_i \parenth{\hat{a}_i\tp \rvg}^2 \parenth{\hat{b}_i\tp \rvg}\leq \tailconstjohn_3 \sqrt{240}\johnkappa\dims^{1/2}} &\geq 1-\frac{\epsilon}{16},
    \label{eq:john_john_cubic_f} \\
%
    \Prob\brackets{\sum_{i=1}^\obs \johnweights_i \parenth{\hat{a}_i\tp \rvg}^4\leq \tailconstjohn_4 \sqrt{1680}\dims} &\geq 1-\frac{\epsilon}{16},
    \label{eq:john_john_fourth} \\
%
    \Prob\brackets{\sum_{i=1}^\obs \johnweights_i \parenth{\hat{a}_i\tp \rvg}^6 \leq \tailconstjohn_6 \sqrt{15120}\dims} &\geq 1-\frac{\epsilon}{16}.
    \label{eq:john_john_sixth}
  \end{align}
  \end{subequations}
\end{lemma}
See Section~\ref{sub:proof_of_lemma_lemma:john_gaussian_moment_bounds} for the proof.
% subsection tail_bounds (end)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Proof of Lemma~\ref{lemma:john_close_hessian_eigenvalues}}
\label{sec:proof_of_lemma_lemma:john_close_hessian_eigenvalues}

  As a direct consequence of Lemma~\ref{lemma:john_closeness_of_slackness}, for any $x, y \in \intP$ such that \mbox{$\vecnorm{x-y}{x} \leq t/\johnkappa^2$}, we have
  \begin{align}
    \label{eq:john_slackness_tbound}
    \max_{i\in[\obs]}\abss{1 - \frac{\slack_{y, i}}{\slack_{x, i}}}
    \leq \frac{2t}{\johnkappa^2}.
  \end{align}
  Bounding the terms in $\hesslogbarr_x$ one by one, we obtain
  \begin{align*}
    \parenth{1 - \frac{2t}{\johnkappa^2}}^2 \hesslogbarr_y
    \preceq \hesslogbarr_x
    \preceq \parenth{1 + \frac{2t}{\johnkappa^2}}^2 \hesslogbarr_y.
  \end{align*}
  We claim that
  \begin{align}
    \label{eq:john_log_weight_final_bound}
    \vecnorm{\log \johnweights_{y} - \log \johnweights_{x}}{\infty} \leq 16 t.
  \end{align}
  Assuming the claim as given at the moment, we now complete the proof.
  Putting the result~\eqref{eq:john_log_weight_final_bound} in matrix form, we obtain that $\exp \parenth{-16t} \Ind_\obs
    \preceq \johnweightmatrix_x^{-1} \johnweightmatrix_y \preceq
    \exp \parenth{ 16t} \Ind_\obs$,
  % \begin{align*}
  %   - 16 t \Ind_\obs
  %   \preceq \log \johnweightmatrix_y - \log \johnweightmatrix_x
  %   \preceq 16 t \Ind_\obs.
  % \end{align*}
  % Thus we can sandwich the matrix $\johnweightmatrix_x^{-1}\johnweightmatrix_y$ as follows
  % \begin{align*}
  %   \exp \parenth{-16t} \Ind
  %   \preceq \johnweightmatrix_x^{-1} \johnweightmatrix_y \preceq
  %   \exp \parenth{ 16t} \Ind,
  % \end{align*}
  and hence
  \begin{align}
    \label{eq:john_bound_on_ratio_of_johnweights}
    \exp \parenth{-16t} \johnweights_{x, i}
    \leq \johnweights_{y, i}
    \leq \exp \parenth{16t} \johnweights_{x, i}.
  \end{align}
  Consequently, using the definition of $\john_x$ we have,
  \begin{align*}
    \underbrace{ \parenth{1 - \frac{2t}{\johnkappa^2}}^2 \exp\parenth{-16t}}_{\omega_\ell} \john_x
    \leq \john_y
    \leq \underbrace{ \parenth{1 + \frac{2t}{\johnkappa^2}}^2 \exp \parenth{16t} }_{\omega_u} \john_y.
  \end{align*}
  Letting $\omega = 2t$, we obtain
  \begin{align*}
    \omega_\ell
     \geq (1-\omega)^2 \cdot \exp\parenth{-8\omega}
    \stackrel{(i)}{\geq} 1-24\omega + \omega^2, \quad \text{ and } \quad
    \omega_u
    \leq (1+\omega)^2 \cdot \exp\parenth{8\omega}
    \stackrel{(ii)}{\leq} 1+24\omega + \omega^2,
  \end{align*}
  where inequalities $(i)$ and $(ii)$ hold since $\omega \leq 1/24$.
  Putting the pieces together, we find that
  \begin{align*}
    \parenth{1-48t+4t^2} \john_x
    \preceq \john_y
    \preceq \parenth{1-48t+4t^2} \john_x
  \end{align*}
  for $t \in [0, 1/48]$.

Now, we return to the proof of our earlier claim~\eqref{eq:john_log_weight_final_bound}.
We use an argument based on the continuity of the function $x \mapsto \log \johnweights_x$.
(Such an argument appeared in a similar scenario in~\cite{lee2014path}.)
For $\lambda \in [0, 1]$, define \mbox{$u_\lambda = \lambda y + \parenth{1- \lambda}x$}.
Let
  \begin{align}
    \label{eq:john_log_weight_initial_bound}
    \lambda^{\mathrm {max}} \defn \sup\braces{\lambda \in [0, 1] \bigg\vert \vecnorm{\log \johnweights_{u_\lambda} - \log \johnweights_x}{\infty} \leq 16 t}.
  \end{align}
  % Note that $\lambda^{\mathrm {max}} \geq 0$.
  It suffices to establish that $\lambda^{\mathrm {max}} = 1$.
  Note that $\lambda = 0$ is feasible on the RHS of equation~\eqref{eq:john_log_weight_initial_bound} and hence $\lambda^{\mathrm {max}}$ exists.
  Now for any $\lambda \in [0, \lambda^{\mathrm {max}}]$ and $i \in \{1, \ldots, \obs\}$, there exists $v$ on the segment $\overline{u_\lambda x}$ such that
  \begin{align*}
    \abss{\log \johnweights_{u_\lambda, i} - \log \johnweights_{x, i}} & = \abss{\parenth{ \frac{\nabla \johnweights_{v, i}}{\johnweights_{v, i}}} \tp \parenth{u_\lambda - x}}
    \stackrel{(i)}{\leq} \vecnorm{ \johnweightmatrix_v^{-1} \johnweightmatrix'_v \parenth{y - x} }{\infty}
    = 2 \vecnorm{\parenth{\johnweightmatrix_v - \alpha\johnlaplacian_v}^{-1} \johnlaplacian_v A_v \parenth{y - x} }{\infty}.
  \end{align*}
  where in step $(i)$ we have used the fact that $u_\lambda - x = \lambda (y-x)$ and $\lambda \in [0, 1]$.
  We claim that
  \begin{align}
    \label{eq:john_step_consistency_infty}
    \vecnorm{\parenth{\johnweightmatrix_v - \alpha\johnlaplacian_v}^{-1} \johnlaplacian_v \myvec_1}{\infty} \leq \johnkappa  \vecnorm{\myvec_1}{\infty} +  2 \johnkappa^2 \vecnorm{\johnweightmatrix_v^{1/2}\myvec_1}{2}
    \quad \mbox{for any $\myvec_1 \in \real^\obs$}.
  \end{align}
  We prove the claim at the end of this section.
  We now derive bounds for the two terms on the RHS of the equation~\eqref{eq:john_step_consistency_infty} for $\myvec_1 = A_v (y-x)$.
  Note that
  \begin{align*}
    \vecnorm{A_v \parenth{y - x}}{\infty} = \max_i  \abss{\frac{\slack_{y, i} - \slack_{x, i}}{\slack_{v, i}}} = \max_i  \abss{\frac{\slack_{y, i} - \slack_{x, i}}{\slack_{x, i}}} \abss{\frac{\slack_{x, i}}{\slack_{v, i}}} \stackrel{(i)}{\leq} \frac{2t}{\johnkappa^2 \parenth{1 - 2t/\johnkappa^2}} \stackrel{(ii)}{\leq} \frac{3t}{\johnkappa^2}.
  \end{align*}
  Inequality $(i)$ uses bound~\eqref{eq:john_slackness_tbound} and inequality $(ii)$ follows by plugging in $t\leq 1/64$.
  Next, we have
  \begin{align*}
    \vecnorm{\johnweightmatrix_v^{1/2}A_v \parenth{y - x}}{2}^2
    % = \sum_{i=1}^\obs \johnweights_{v,i} \frac{\parenth{a_i \tp \parenth{y - x}}^2}{\slack_{v,i}^2}
    = \sum_{i=1}^\obs \johnweights_{x,i} \frac{\parenth{a_i \tp \parenth{y - x}}^2}{\slack_{x,i}^2} \frac{\johnweights_{v, i}}{\johnweights_{x, i}} \frac{\slack_{v, i}^2}{\slack_{x, i}^2}
    & \stackrel{(i)}{\leq} \vecnorm{x - y}{x}^2 \ \max_{i \in [\obs]} \frac{\johnweights_{v, i}}{\johnweights_{x, i}} \frac{\slack_{v, i}^2}{\slack_{x, i}^2} \\
    & \stackrel{(ii)}{\leq} \frac{t^2}{\johnkappa^4} \parenth{1 + (16t) +(16t)^2} \parenth{1 + \frac{2t}{\johnkappa^2}}^2 \\
    & \stackrel{(iii)}{\leq} \frac{1.5 t}{\johnkappa^4},
  \end{align*}
  where step $(i)$ follows from the definition of the local norm; step $(ii)$ follows from bounds~\eqref{eq:john_slackness_tbound} and \eqref{eq:john_log_weight_initial_bound} and the fact that $e^x \leq 1+ x + x^2 $ for all $x \in [0, 1/4]$; and inequality $(iii)$ follows by plugging in $t\leq 1/64$.
  Putting the pieces together, we obtain
  \begin{align*}
    \vecnorm{\log \johnweights_{u_\lambda} - \log \johnweights_{x}}{\infty} \leq 2(\johnkappa\cdot 3t/\johnkappa^2 + 2 \johnkappa^2 \cdot 1.5t/\johnkappa^4 ) \leq 12 t < 16 t.
  \end{align*}
  The strict inequality is valid for $\lambda = \lambda^{\mathrm {max}}$.
  Consequently, using the continuity of $x \mapsto \log \johnweights_x$, we conclude that $\lambda^{\mathrm {max}} = 1$.

 It is left to prove claim~\eqref{eq:john_step_consistency_infty}.
 Let $\myvectwo \defn \parenth{\johnweightmatrix_v - \alpha\johnlaplacian_v}^{-1} \johnlaplacian_v \myvec_1$.
  % \begin{align*}
  %   z = \parenth{\johnweightmatrix_v - \alpha\johnlaplacian_v}^{-1} \johnlaplacian_v p.
  % \end{align*}
  which implies $\parenth{\johnweightmatrix_v - \alpha\johnlaplacian_v} \myvectwo = \johnlaplacian_v \myvec_1$.
  % \begin{align*}
  %   \parenth{\johnweightmatrix_v - \alpha\johnlaplacian_v} z = \johnlaplacian_v p.
  % \end{align*}
  Plugging the expression of $\johnweightmatrix_v$ and $\johnlaplacian_v$, we have
  \begin{align*}
    \parenth{(1-\alpha)\johnlevmatrix_v + \johnbeta\Ind_\obs + \alpha \johnprojmatrix_v^{(2)}} \myvectwo = \parenth{\johnlevmatrix_v - \johnprojmatrix_v^{(2)}} \myvec_1.
  \end{align*}
  Writing component wise, we find that for any $i \in [\obs]$, we have
  \begin{align}
    \abss{\parenth{(1-\alpha)\levjohn_{v,i} + \johnbeta} \myvectwo_i}
    &\leq \alpha \abss{e_i\tp\johnprojmatrix_v^{(2)} \myvectwo } +  \levjohn_{v,i} \abss{\myvec_{1, i}} + \abss{e_i\tp\johnprojmatrix_v^{(2)} \myvec_1} \notag\\
    & \stackrel{(i)}{\leq} \alpha \levjohn_{v, i} \vecnorm{\johnlevmatrix_v^{1/2} \myvectwo}{2} +  \levjohn_{v,i} \vecnorm{\myvec_1}{\infty} + \levjohn_{v, i} \vecnorm{\johnlevmatrix_v^{1/2} \myvec_1}{2} \notag\\
    & \stackrel{(ii)}{\leq} \alpha \levjohn_{v, i} \vecnorm{\johnweightmatrix_v^{1/2} \myvectwo}{2} +  \levjohn_{v,i} \vecnorm{\myvec_1}{\infty} + \levjohn_{v, i} \vecnorm{\johnweightmatrix_v^{1/2} \myvec_1}{2} \notag\\
    & \stackrel{(iii)}{\leq} \alpha \levjohn_{v, i} \johnkappa \vecnorm{\johnweightmatrix_v^{1/2} \myvec_1}{2} +  \levjohn_{v,i} \vecnorm{\myvec_1}{\infty} + \levjohn_{v, i} \vecnorm{\johnweightmatrix_v^{1/2} \myvec_1}{2},
    \label{eq:john_final_infty_two_bound}
  \end{align}
  where inequality $(ii)$ from the fact that $\johnlevmatrix_y \preceq \johnweightmatrix_y$ and inequality $(iii)$ from Lemma~\ref{lemma:f_to_d_l2} with $c_1=0, c_2 = 1$.
  To assert inequality $(i)$, observe the following
  \begin{align*}
    \abss{\sum_{j=1}^\obs \levjohn_{y, i, j}^2 \myvectwo_j}
    \leq \sum_{j=1}^\obs \levjohn_{y, i, j}^2 \abss{\myvectwo_j}
    \stackrel{(a)}{\leq} \levjohn_{y, i} \sum_{j=1}^\obs \levjohn_{y, j} \abss{\myvectwo_j}
    \stackrel{(b)}{\leq} \levjohn_{y, i} \sum_{j=1}^\obs \sqrt{\levjohn_{y, j}} \abss{\myvectwo_j}
    = \levjohn_{y, i} \vecnorm{\johnlevmatrix_v^{1/2}\myvectwo}{2},
  \end{align*}
  where step $(a)$ follows from the fact that $\levjohn_{y, i, j}^2 \leq \levjohn_{y, i} \levjohn_{y, j}$, and step $(b)$ from the fac that $\levjohn_{y, i} \in [0 ,1]$.
  Dividing both sides of inequality~\eqref{eq:john_final_infty_two_bound} by $\parenth{(1-\alpha)\levjohn_{v,i} + \johnbeta}$ and observing that $\levjohn_{v, i}/\parenth{(1-\alpha)\levjohn_{v,i} + \johnbeta} \leq\johnkappa$, and $\alpha \in [0, 1]$, yields the claim.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Proof of Lemma~\ref{lemma:john_change_in_log_det_and_local_norm}} % (fold)
\label{sec:proof_of_lemma_lemma:john_change_in_log_det_and_local_norm}

We prove Lemma~\ref{lemma:john_change_in_log_det_and_local_norm} in two parts: claim~\eqref{eq:john_whp_log_det_filter} in Section~\ref{ssec:proof_of_claim_whp_log_det_filter} and claim~\eqref{eq:john_whp_local_norm} in Section~\ref{ssec:proof_of_claim_whp_local_norm}.
\subsection{Proof of claim~\eqref{eq:john_whp_log_det_filter}}
\label{ssec:proof_of_claim_whp_log_det_filter}
Using the second order Taylor expansion, we have
\begin{align*}
  \logdetJ_z - \logdetJ_x
  = \parenth{z - x}\tp \gradlogdetJ_x + \frac{1}{2} \parenth{z - x}\tp \hesslogdetJ_y \parenth{z - x},
  \quad \mbox{for some $y \in \overline{xz}$}.
\end{align*}
We claim that for $r\leq \johnradiusbound(\epsilon)$, we have
\begin{subequations}
  \label{eq:john_log_det_two_tails}
  \begin{align}
    \Prob \brackets{ \parenth{z-x}\tp \gradlogdetJ_x \geq -
      \epsilon/2} &\geq 1 - \epsilon/2,
    \ \text{and} \label{eq:john_gradient_log_det_tail} \\
    \quad \Prob
    \brackets{ {\frac{1}{2} \parenth{z-x} \hesslogdetJ_y
        \parenth{z-x}} \geq -\epsilon/2} &\geq 1 - \epsilon/2. \label{eq:john_hessian_log_det_tail}
  \end{align}
\end{subequations}
Note that the claim~\eqref{eq:john_whp_log_det_filter} follows from the above two claims.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Proof of bound~(\ref{eq:john_gradient_log_det_tail})}
\label{sssec:proof_of_claim_eq_gradient_log_det_tail}

We observe that
\begin{align*}
  \parenth{z - x}\tp \nabla \logdetJ_x \sim \NORMAL \parenth{0, \frac{r^2}{\johnkappa^2 n} \nabla \logdetJ_x\tp \john_x^{-1} \nabla \logdetJ_x}.
\end{align*}
Let $\theinverse_x = \Ind_\obs + \parenth{\johnweightmatrix_x - \alpha\johnlaplacian_x}^{-1} \johnlaplacian_x$.
Substituting the expression of $\gradlogdetJ_x$ from Lemma~\ref{lemma:john_gradient_and_hessian_and_bounds}~\ref{item:gradient_log_det} and applying Cauchy-Schwarz inequality, we have that for any vector $\myvec \in \real^\dims$
\begin{align}
  \myvec\tp \nabla \logdetJ_x \nabla \logdetJ_x \tp \myvec
  % & = \angles{\myvec, A_x\tp \parenth{\Ind + \johnlaplacian_x \theinverse_x} \johnweightmatrix_x \johnlocalslack_x}^2
  = (\johnlocalslack_x\tp \johnweightmatrix_x \theinverse_x A_x \myvec)^2
  \leq \parenth{\myvec \tp A_x\tp \johnweightmatrix_x A_x \myvec} \cdot
  \parenth{\johnlocalslack_x \tp \johnweightmatrix_x  \theinverse_x \johnweightmatrix_x^{-1} \theinverse_x \johnweightmatrix_x \johnlocalslack_x}.  \label{eq:john_gradient_log_det_variance_bound}
\end{align}
Observe that
\begin{align*}
  \johnweightmatrix_x^{1/2}\theinverse_x\johnweightmatrix_x^{-1/2} = \Ind_\obs + (\Ind_\obs - \alpha \johnweightmatrix_x^{-1/2}\johnlaplacian_x\johnweightmatrix_x^{-1/2})^{-1}(\johnweightmatrix_x^{-1/2}\johnlaplacian_x\johnweightmatrix_x^{-1/2}).
\end{align*}
Now, using the intermediate bound~\eqref{eq:john_G_laplace_G_bound} from the proof of Lemma~\ref{lemma:f_to_d_l2}, we obtain that
\begin{align*}
  \Ind_\obs \preceq \johnweightmatrix_x^{1/2}\theinverse_x\johnweightmatrix_x^{-1/2} \preceq 2\johnkappa\Ind_\obs,
\end{align*}
and hence $\johnweightmatrix_x \preceq \johnweightmatrix_x  \theinverse_x \johnweightmatrix_x^{-1} \theinverse_x \johnweightmatrix_x \preceq 4 \johnkappa^2 \johnweightmatrix_x$.
% \begin{align*}
%   \Ind_\obs \preceq \johnweightmatrix_x  \theinverse_x \johnweightmatrix_x^{-1} \theinverse_x \johnweightmatrix_x \preceq 4 \johnkappa^2 \Ind.
% \end{align*}
Consequently, we have
\begin{align*}
  \johnlocalslack_x \tp \johnweightmatrix_x  \theinverse_x \johnweightmatrix_x^{-1} \theinverse_x \johnweightmatrix_x \johnlocalslack_x
  \leq 4\johnkappa^2 \johnlocalslack_x\tp \johnweightmatrix_x \johnlocalslack_x = 4\johnkappa^2 \sum_{i=1}^\obs \johnweights_{x, i} \johnlocalslack_{x, i}^2 \leq 16 \johnkappa^2 \dims,
\end{align*}
where the last step follows from Lemma~\ref{ppt:john_all_properties}.
Putting the pieces together into equation~\eqref{eq:john_gradient_log_det_variance_bound}, we obtain $\gradlogdetJ_x \gradlogdetJ_x\tp \preceq 16 \johnkappa^2 \dims \john_x$ whence
$\john_x^{-1/2} \gradlogdetJ_x \gradlogdetJ_x\tp \john_x^{-1/2} \preceq 16 \johnkappa^2 \dims \Ind_\dims$.
Noting that the matrix $\john_x^{-1/2} \gradlogdetJ_x \gradlogdetJ_x\tp \john_x^{-1/2}$ has rank one, we have
\begin{align*}
  \gradlogdetJ_x\tp \john_x^{-1} \gradlogdetJ_x = \trace \parenth{\john_x^{-1/2} \gradlogdetJ_x  \gradlogdetJ_x\tp \john_x^{-1/2}} \leq 16 \johnkappa^2 \dims.
\end{align*}
Using standard Gaussian tail bound, we have $\Prob\parenth{\parenth{z-x}\tp \gradlogdetJ_x  \geq -\sqrt{32}\tailconstjohn_1 r} \geq 1 - \exp\parenth{-\tailconstjohn_1^2}.$

Choosing $\tailconstjohn_1 = \log(2/\epsilon)$, and observing that
\begin{align}
  \label{eq:john_gradient_log_det_tail_r_condition}
  r \leq \frac{\epsilon}{\parenth{2\sqrt{32}\tailconstjohn_1}},
\end{align}
yields the claim.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Proof of bound~(\ref{eq:john_hessian_log_det_tail})}
\label{sssec:proof_of_claim_eq_hessian_log_det_tail}
In the following proof, we use $h = z-x$ for definitions~\eqref{eq:john_def_D}-\eqref{eq:john_def_rho}.
According to Lemma~\ref{lemma:john_gradient_and_hessian_and_bounds}\ref{item:john_hessian_log_det_bound}, we have
\begin{align*}
  \abss{\frac{1}{2} \parenth{z - x}\tp \hesslogdetJ_y \parenth{z - x}}
  \leq  \sum_{i=1}^\obs \johnweights_{y, i}\, \johnlocalslack_{y, i} \brackets{ \frac{9}{2} \, \projd_{y, i}^2 + 2 \projf_{y, i}^2}   +  \frac{1}{2}\abss{ \sum_{i=1}^\obs \johnweights_{y, i}\, \johnlocalslack_{y, i} \projz_{y, i}}
\end{align*}
We claim that
\begin{align}
  \sum_{i=1}^\obs \johnweights_{y, i}\, \johnlocalslack_{y, i} \brackets{ \frac{9}{2} \, \projd_{y, i} ^2 + 2 \projf_{y, i}^2}   +  \frac{1}{2}\abss{ \sum_{i=1}^\obs \johnweights_{y, i}\, \johnlocalslack_{y, i} \projz_{y, i}}
  \leq 386 \sqrt{\dims} \johnkappa^4  \sum_{i=1}^\obs \johnweights_{y, i}  \projd_{y, i}^2.
  \label{eq:john_hess_logdet_in_terms_of_d}
\end{align}
Assuming the claim as given at the moment, we now complete the proof.
Note that $y$ is some particular point on $\overline{xz}$ and its dependence on $z$ is hard to characterize.
Consequently, we transfer all the terms with dependence on $y$, to terms with dependence on $x$ only.
We have
\begin{align*}
  \sum_{i=1}^\obs \johnweights_{y, i} \projd_{y, i}^2 = \sum_{i=1}^\obs \johnweights_{x, i} \projd_{x, i}^2 \underbrace{\frac{\johnweights_{y, i}}{\johnweights_{x, i}} \frac{s_{x, i}^2}{s_{y, i}^2}}_{\tau_{y, i}}.
\end{align*}
We now invoke the following high probability bounds implied by Lemma~\ref{lemma:john_whp_slackness} and Lemma~\ref{lemma:john_gaussian_moment_bounds}~\eqref{eq:john_john_quadratic} respectively
\begin{align}
  \Prob\brackets{\sup_{y \in\overline{xz}, i \in [\obs]}\tau_{y, i} \leq 1.1} \geq 1-\epsilon/4,
  \quad \text{and}, \quad
  \Prob\brackets{\sum_{i=1}^\obs \johnweights_{x, i}  \parenth{\hat{a}_{x, i}\tp \rvg}^2 \leq \tailconstjohn_2 \sqrt{24}\dims} \geq 1-\epsilon/16.
  \label{eq:john_hbp_logdetjohn}
\end{align}
Since $h = z-x$, we have that $\projd_{x, i}^2 = \frac{r^2}{\johnkappa^2 \dims^{3/2}}\parenth{\hat{a}_{x,i}\tp \rvg}^2$.
Consequently, for
\begin{align}
  \label{eq:john_hessian_log_det_tail_r_condition}
  r \leq \sqrt{\frac{\epsilon}{386\sqrt{24}\tailconstjohn_2}},
\end{align}
with probability at least $1-\epsilon/2$, we have
\begin{align*}
  \abss{\frac{1}{2} \parenth{z - x}\tp \hesslogdetJ_y \parenth{z - x}}
  \stackrel{\mathrm{eqn.}~\eqref{eq:john_hess_logdet_in_terms_of_d}}{\leq} 386 \sqrt{\dims} \johnkappa^4  \sum_{i=1}^\obs \johnweights_{y, i}  \projd_{y, i}^2
  \stackrel{\mathrm{hpb}~\eqref{eq:john_hbp_logdetjohn}}{\leq} \epsilon,
\end{align*}
which completes the proof.

We now turn to the proof of claim~\eqref{eq:john_hess_logdet_in_terms_of_d}.
First we observe the following relationship between the terms $\projd_{y, i}$ and  $\projf_{y, i}$:
\begin{align}
  \sum_{i=1}^\obs\! \johnweights_{y, i} \projf_{y, i}^2
  \!\stackrel{(i)}{=} \! 4 h\tp A_y\tp \!\Lambda_y \parenth{\johnweightmatrix_y \!-\! \alpha \johnlaplacian_y}^{-1}\! \johnweightmatrix_y \parenth{\johnweightmatrix_y\! -\! \alpha \johnlaplacian_y}^{-1} \!\johnlaplacian_y A_y h \!
  \stackrel{(ii)}{\leq}\! 4 \johnkappa^2 h\tp\! A_y\tp\!  \johnweightmatrix_y A_y h
   \!=\! 4 \johnkappa^2 \sum_{i=1}^\obs \johnweights_{y, i} \projd_{y, i}^2,
  \label{eq:john_exact_f_to_d_bound}
\end{align}
where step $(i)$ follows by plugging in the definition of $\projf_{y, i}$~\eqref{eq:john_def_F} and step~$(ii)$ by invoking Lemma~\ref{lemma:f_to_d_l2} with $c_1 =0 $ and $c_2 = 1$.
Next, we relate the term on the LHS of equation~\eqref{eq:john_hess_logdet_in_terms_of_d} involving $\projz_{y, i}$ to a polynomial in $\projd_{y, i}$.
Using Lemma~\ref{lemma:john_gradient_and_hessian_and_bounds}, we find that
\begin{align*}
\abss{ \sum_{i=1}^\obs \johnweights_{y, i}\, \johnlocalslack_{y, i} \projz_{y, i}}
&= \abss{\parenth{\parenth{\johnweightmatrix_y - \alpha \johnlaplacian_y}^{-1} \johnweightmatrix_y \theta_y}\tp \parenth{\johnweightmatrix_y - \alpha \johnlaplacian_y} \projz_y}
\leq \vecnorm{\underbrace{\parenth{\johnweightmatrix_y - \alpha \johnlaplacian_y}^{-1} \johnweightmatrix_y \theta_y}_{v_1}}{\infty}
\vecnorm{\underbrace{\parenth{\johnweightmatrix_y - \alpha \johnlaplacian_y} \projz_y}_{\projzsub_y}}{1},
\end{align*}
where the last step follows from the Holder's inequality: for any two vectors $u, v \in \realdim$, we have that $u\tp v \leq \vecnorm{u}{\infty} \vecnorm{v}{1}$.
Substituting the bound for the norm $\vecnorm{v_1}{\infty}$ from Corollary~\ref{corollary:f_to_d_l1} and the bound on $\projzsub_{y, i}$ from Lemma~\ref{lemma:john_gradient_and_hessian_and_bounds}\ref{item:hessian_g}, we obtain that
% \begin{align*}
% \vecnorm{\parenth{\johnweightmatrix_y - \alpha \johnlaplacian_y}^{-1} \johnweightmatrix_y \theta_y}{\infty} \leq 3 \sqrt{\dims} \johnkappa^{3/2} \vecnorm{\theta_y}{\infty} \leq 12 \sqrt{\dims} \johnkappa^{3/2}.
% \end{align*}
\begin{align*}
  \abss{ \sum_{i=1}^\obs \johnweights_{y, i}\, \johnlocalslack_{y, i} \projz_{y, i}}
  % & \leq 12 \sqrt{n} \johnkappa^{3/2} \vecnorm{\parenth{\johnweightmatrix_y - \alpha \johnlaplacian_y} \projz_y}{1} \\
  \!\leq 12 \sqrt{n} \johnkappa^{3/2} \sum_{i=1}^\obs \bigg[{7 \johnweights_{y, i} \projd_{y, i}^2 \!+\! 3 \johnweights_{y, i} \projf_{y, i}^2 \!+\! \sum_{j=1}^\obs \parenth{ 13\projd_{y, j}^2 \!+\! 6 \projf_{y, j}^2} \johnprojmatrix_{y, i, j}^2}\bigg]
  \!\leq\! 672\sqrt{n} \johnkappa^{4} \sum_{i=1}^\obs \johnweights_{y, i} \projd_{y, i}^2,
\end{align*}
where the last step follows from Lemma~\ref{ppt:john_all_properties}\ref{item:john_sigma_properties} and the bound~\eqref{eq:john_exact_f_to_d_bound}.
The claim now follows.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of claim~(\ref{eq:john_whp_local_norm})}
\label{ssec:proof_of_claim_whp_local_norm}

Writing $z = x + t u$, where $t$ is a scalar and $u$ is
a unit vector in \realdim, we obtain
\begin{align*}
\vecnorm{z-x}{z}^2 - \vecnorm{z-x}{x}^2 = t^2 \sum_{i=1}^\obs
\parenth{a_i\tp u}^2 \parenth{\johnphi_{z, i} - \johnphi_{x, i}}.
\end{align*}
Now, we use a Taylor series expansion for $\sum_{i=1}^\obs
\parenth{a_i\tp u}^2 \parenth{\johnphi_{z, i} - \johnphi_{x, i}}$ around
the point $x$, along the line $u$.  There exists a point $y \in
\overline{xz}$ such that
\begin{align*}
\sum_{i=1}^\obs \parenth{a_i\tp u}^2 \parenth{\johnphi_{z, i} -
  \johnphi_{x, i}} = \sum_{i=1}^\obs \parenth{a_i\tp u}^2 \parenth{
  \parenth{z - x}\tp \nabla \johnphi_{x, i}+ \frac{1}{2}
  \parenth{z-x}\tp \nabla^2 \johnphi_{y, i} \parenth{z-x}}.
\end{align*}
Note that the point $y$ in this discussion is not the same as the point $y$ used in previous proofs, in particular in Section~\ref{ssec:proof_of_claim_whp_log_det_filter}.
% This notation does not cause confusion as the following results hold for any $y$ on the segment $\overline{xz}$.
Multiplying both sides by $t^2$, and using the shorthand
$\projd_{x, i} = \frac{a_i\tp (z-x)}{\slack_{x,i}}$, we obtain
\begin{align}
  \label{eq:john_z_x_two_terms}
\vecnorm{z \!-\! x}{z}^2 \!-\! \vecnorm{z\!-\!x}{x}^2 &=
\sum_{i=1}^\obs \projd_{x, i}^2 \slack_{x, i}^2 \parenth{z\!-\!x}\tp
\nabla \johnphi_{x, i} + \sum_{i=1}^\obs \projd_{x, i}^2 \slack_{x, i}^2
\frac{1}{2} \parenth{z\!-\!x}\tp \nabla^2 \johnphi_{y, i}
\parenth{z\!-\!x}.
\end{align}
We claim that for $r\leq \johnradiusbound(\epsilon)$, we have
\begin{subequations}
    \label{eq:john_local_norm_two_tails}
    \begin{align}
        \Prob_{z \sim \transition^\tagjohn_x} \brackets{ \sum_{i=1}^\obs \projd_{x, i}^2 \slack_{x, i}^2 \parenth{z\!-\!x}\tp
\nabla \johnphi_{x, i} \leq
          \epsilon \frac{r^2}{\johnkappa^4 \dims^{3/2}}} &\geq 1 - \epsilon/2,
        \ \text{and} \label{eq:john_gradient_local_norm_tail} \\
        \quad \Prob_{z \sim \transition^\tagjohn_x}
        \brackets{ \sup_{y \in \overline{xz}} \parenth{\sum_{i=1}^\obs \projd_{x, i}^2 \slack_{x, i}^2
\frac{1}{2} \parenth{z\!-\!x}\tp \nabla^2 \johnphi_{y, i}
\parenth{z\!-\!x}} \leq \epsilon \frac{r^2}{\johnkappa^4 \dims^{3/2}} } &\geq 1 - \epsilon/2. \label{eq:john_hessian_local_norm_tail}
    \end{align}
\end{subequations}
We now prove each claim separately.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Proof of bound~(\ref{eq:john_gradient_local_norm_tail})}
\label{sssec:proof_of_claim_eq_gradient_local_norm_tail}
Using Lemma~\ref{lemma:john_gradient_and_hessian_and_bounds}\ref{item:gradient_phi} and using $h = z-x$ where $z$ is given by the relation~\eqref{eq:john_z_x_relation}, we find that
\begin{align}
\sum_{i=1}^\obs \projd_{x, i}^2 \slack_{x, i}^2 \parenth{z\!-\!x}\tp \nabla \johnphi_{x, i}
&= \sum_{i=1}^\obs \johnweights_{x, i} \projd_{x, i}^2  \parenth{2 \projd_{x, i} + \projf_{x, i}}\notag\\
&= \frac{r^3}{\dims^{9/4} \johnkappa^6} \sum_{i=1}^\obs \johnweights_{x, i} \parenth{\hat{a}_{x,i} \tp \xi}^3
  + \frac{2r^3}{\dims^{9/4} \johnkappa^6} \sum_{i=1}^\obs \johnweights_{x, i} \parenth{\hat{a}_{x,i} \tp \xi}^2 \parenth{\hat{b}_{x,i} \tp \xi}
  \label{eq:john_two_terms_gradient_phi}
\end{align}
Using high probability bounds for the two terms in equation~\eqref{eq:john_two_terms_gradient_phi} from Lemma~\ref{lemma:john_gaussian_moment_bounds}, part~\eqref{eq:john_john_cubic} and part~\eqref{eq:john_john_cubic_f},  we obtain that
\begin{align*}
  \abss{\sum_{i=1}^\obs \projd_{x, i}^2 \slack_{x, i}^2 \parenth{z\!-\!x}\tp
  \nabla \johnphi_{x, i}}
  \leq \frac{5 \sqrt{60} \tailconstjohn_3 r^3}{\johnkappa^5\dims^{7/4}}
  \leq \epsilon \frac{r^2}{\johnkappa^4\dims^{3/2}},
\end{align*}
with probability at least $1 - \epsilon/2$.
The last inequality uses the condition that
\begin{align}
  \label{eq:john_gradient_local_norm_tail_r_condition}
  r \leq \frac{\epsilon}{5\sqrt{60} \tailconstjohn_3}.
\end{align}
The claim now follows.
\subsubsection{Proof of bound~(\ref{eq:john_hessian_local_norm_tail})}
\label{sssec:proof_of_claim_eq_hessian_local_norm_tail}
Note that $\projd_{x, i}\slack_{x, i} = a_i\tp h = \projd_{y, i} \slack_{y, i}$ for any $h$.
Using this equality for $h = z-x$, we find that
\begin{align}
    \abss{\sum_{i=1}^\obs \projd_{x, i}^2 \slack_{x, i}^2 \frac{1}{2} h\tp \nabla^2 \johnphi_{y, i} h}
    & = \abss{\sum_{i=1}^\obs \projd_{y, i}^2 \slack_{y, i}^2 \frac{1}{2} h\tp \nabla^2 \johnphi_{y, i} h} \notag\\
    & \stackrel{(i)}{\leq} 3 \underbrace{\sum_{i=1}^\obs \johnweights_{y, i} \projd_{y, i}^4}_{C_1} + 2\underbrace{\abss{\sum_{i=1}^\obs \johnweights_{y,i} \projd_{y, i}^3 \projf_{y, i}}}_{C_2} + \underbrace{\abss{\sum_{i=1}^\obs \johnweights_{y, i} \projd_{y, i}^2 \projz_{y, i}}}_{C_3}, \label{eq:john_hess_phi_decomposition}
\end{align}
where step~$(i)$ follows from Lemma~\ref{lemma:john_gradient_and_hessian_and_bounds}\ref{item:hessian_beta_bound}.
We can write $C_1$ as follows
\begin{align}
\sum_{i=1}^\obs \johnweights_{y, i} \projd_{y, i}^4
 = \sum_{i=1}^\obs \johnweights_{x, i} \projd_{x, i}^4 \frac{\johnweights_{y, i}}{\johnweights_{x, i}} \frac{\projd_{y, i}^4}{\projd_{x, i}^4}
 = \frac{r^4}{n^3 \johnkappa^8}  \sum_{i=1}^\obs \johnweights_{x, i} \parenth{\hat{a}_{x, i}\tp \rvg}^4 \frac{\johnweights_{y, i}}{\johnweights_{x, i}} \frac{\projd_{y, i}^4}{\projd_{x, i}^4}.
 \label{eq:john_hess_phi_c1}
\end{align}
Now, we claim the following:
\begin{subequations}
\begin{align}
  C_2 &\leq 2 \frac{r^4}{n^3 \johnkappa^7}  \cdot \sqrt{\brackets{ \sum_{i=1}^\obs \johnweights_{x, i} \parenth{\hat{a}_{x, i}\tp \rvg}^2 \frac{\johnweights_{y, i}}{\johnweights_{x, i}} \frac{\projd_{y, i}^2}{\projd_{x, i}^2}}
  \cdot
  \brackets{\sum_{i=1}^\obs \johnweights_{x, i} \parenth{\hat{a}_{x,i}\tp \rvg}^6 \frac{\johnweights_{y, i}}{\johnweights_{x, i}} \frac{\projd_{y, i}^6}{\projd_{x, i}^6}}}, \quad \text{and}, \label{eq:john_C2_hess_phi}\\
  % C_3 &\leq 164 \parenth{\sum_{i=1}^\obs \johnweights_{x, i} \projd_{x, i}^2 \frac{\johnweights_{y, i}}{\johnweights_{x, i}} \frac{\projd_{y, i}^2}{\projd_{x, i}^2}} \parenth{\johnkappa\max_i \projd_{y, i}^2 + \sqrt{\johnkappa^3 \sum_{i=1}^\obs \johnweights_{x, j} \projd_{x, j}^4 \frac{\johnweights_{y, i}}{\johnweights_{x, i}} \frac{\projd_{y, i}^4}{\projd_{x, i}^4} }}\\
  C_3 &\leq 56 \frac{r^4}{n^3 \johnkappa^{4.5}} \parenth{\sum_{i=1}^\obs \johnweights_{x, i} \parenth{\hat{a}_{x, i}\tp \rvg}^2 \frac{\johnweights_{y, i}}{\johnweights_{x, i}} \frac{\projd_{y, i}^2}{\projd_{x, i}^2}} \parenth{\max_i \parenth{\hat{a}_{x, i}\tp \rvg}^2 \frac{\projd_{y, i}^2}{\projd_{x, i}^2}
  + \sqrt{ \sum_{i=1}^\obs \johnweights_{x, i} \parenth{\hat{a}_{x, i}\tp \rvg}^4 \frac{\johnweights_{y, i}}{\johnweights_{x, i}} \frac{\projd_{y, i}^4}{\projd_{x, i}^4} } } \label{eq:john_C3_hess_phi}
\end{align}
\end{subequations}
Assuming the claims as given, we now complete the proof.
Using Lemma~\ref{lemma:john_whp_slackness}, we have
\begin{align*}
\Prob\brackets{\frac{\johnweights_{y, i}}{\johnweights_{x, i}} \frac{\projd_{y, i}^6}{\projd_{x, i}^6} \leq 1.2} \geq 1-\epsilon/4,
\end{align*}
and consequently
\begin{align}
  3C_1 \!+\! 2C_2 \!+\! C_3
  &\leq \frac{r^4}{\dims^3 \johnkappa^{4.5}}
        \Bigg[
        4 \cdot \sum_{i=1}^\obs \johnweights_{x, i} (\hat{a}_{x, i}\tp \rvg)^4
        +10  \cdot \bigg(\sum_{i=1}^\obs \johnweights_{x, i} (\hat{a}_{x, i}\tp \rvg)^2
                              \cdot
                              \sum_{i=1}^\obs \johnweights_{x, i} (\hat{a}_{x,i}\tp \rvg)^6
                    \bigg)^{1/2}
            \notag        \\
  & \quad \quad \quad
        + 100
        \cdot
        {\sum_{i=1}^\obs \johnweights_{x, i} \parenth{\hat{a}_{x, i}\tp \rvg}^2}
        \cdot
        \bigg({
        \max_i ({\hat{a}_{x, i}\tp \rvg})^2
        + \big({ \sum_{i=1}^\obs \johnweights_{x, i} ({\hat{a}_{x, i}\tp \rvg})^4}\big)^{1/2}
        }\bigg)
        \Bigg],
        \label{eq:john_3c1_c2_c3}
\end{align}
with probability at least $1-\epsilon/4$.
Now, we observe that for all $i \in [\obs]$ and $x \in \intP$, we have
\begin{align*}
  \parenth{\hat{a}_{x, i}\tp \rvg} \sim \NORMAL(0, \johnlocalslack_{x, i}) \quad \text{and} \quad \johnlocalslack_{x, i} \leq 4.
\end{align*}
Invoking the standard tail bound for maximum of Gaussian random variables, we obtain
% \begin{align*}
%   \Prob \brackets{\max_i \abss{\parenth{\hat{a}_{x, i}\tp \rvg}} \leq 4\sqrt{\log \obs} \cdot \parenth{2+\sqrt{\log(16/\epsilon)}} } \geq 1 - \epsilon/16.
% \end{align*}
\begin{align*}
  \Prob \brackets{\max_i \abss{\parenth{\hat{a}_{x, i}\tp \rvg}} \leq 8 \cdot \parenth{\sqrt{\log \obs}+\sqrt{\log(32/\epsilon)}} } \geq 1 - \epsilon/16.
\end{align*}
Using the fact that $2c_1c_2 \geq c_1 + c_2$ for all $c_1, c_2 \geq 1$, we obtain
\begin{align*}
   \Prob \brackets{\max_i \abss{\parenth{\hat{a}_{x, i}\tp \rvg}} \leq 16 \cdot{\sqrt{\log \obs} \cdot \sqrt{\log(32/\epsilon)}} } \geq 1 - \epsilon/16.
\end{align*}
Combining this bound with the tail bounds for various Gaussian polynomials~\eqref{eq:john_john_quadratic}, \eqref{eq:john_john_fourth}, \eqref{eq:john_john_sixth} from  Lemma~\ref{lemma:john_gaussian_moment_bounds}, and substituting in inequality~\eqref{eq:john_3c1_c2_c3}, we obtain that
\begin{multline*}
  \abss{\sum_{i=1}^\obs \projd_{x, i}^2 \slack_{x, i}^2 \frac{1}{2} h\tp \nabla^2 \johnphi_{y, i} h}
  \leq \frac{r^4}{\johnkappa^{6.5} \dims^3} \Bigg[ 4\cdot  \tailconstjohn_4\sqrt{1680}\dims + 10 \parenth{\tailconstjohn_2 \sqrt{24}\dims \cdot \tailconstjohn_6 \sqrt{15120} \dims}^{1/2} \\
  + 100 \cdot \tailconstjohn_2 \sqrt{24}\dims\cdot \parenth{256 \cdot \log\obs \cdot \log(32/\epsilon)  + \parenth{\tailconstjohn_4\sqrt{1680}\dims}^{1/2}}\Bigg]
  % &\leq
\end{multline*}
with probability at least $1-\epsilon/2$.
In the above expression, the terms $\tailconstjohn_i$ are a function of $\epsilon$ as defined in Lemma~\ref{lemma:john_gaussian_moment_bounds}.
In particular, $\tailconstjohn_{i} = \tailconstjohn_{i, \epsilon} =  (2e/i \cdot \log(16/\epsilon))^{i/2}$ for $i \in \{2, 3, 4, 6\}$.
Observing that $256 \log(32/\epsilon) \geq \parenth{\tailconstjohn_4 \sqrt{1680}}^{1/2}$, and that our choice of $r$ satisfies
\begin{align}
  \label{eq:john_hessian_local_norm_tail_r_condition}
  r^2 \leq \min\braces{{\frac{\epsilon}{8\sqrt{1680} \tailconstjohn_4}}, {\frac{\epsilon}{40\parenth{\tailconstjohn_2\tailconstjohn_6 \sqrt{24}\sqrt{15120}}^{1/2}}}, {\frac{\epsilon}{204800\tailconstjohn_2\sqrt{24}\log(32/\epsilon)}}},
\end{align}
we obtain
\begin{align*}
  \abss{\sum_{i=1}^\obs \projd_{x, i}^2 \slack_{x, i}^2 \frac{1}{2} h\tp \nabla^2 \johnphi_{y, i} h}
  \leq
  \frac{r^2}{\johnkappa^4 \dims^{3/2}}\brackets{\frac{\epsilon}{2}+ \frac{\epsilon}{4} + \frac{\epsilon}{8}\parenth{ \frac{\log \obs}{\sqrt{\dims}}+1}}.
\end{align*}
Asserting the additional condition $\sqrt{\dims} \geq \log{\obs}$, yields the claim.

It is now left to prove the bounds~\eqref{eq:john_C2_hess_phi} and \eqref{eq:john_C3_hess_phi}.
We prove these bounds separately.
\paragraph{Bounding $C_2$:} % (fold)
\label{par:bounding_c_2}

Applying Cauchy-Schwarz inequality, we have
\begin{align*}
\abss{\sum_{i=1}^\obs \johnweights_{y,i} \projd_{y, i}^3 \projf_{y, i}} \leq \parenth{ \sum_{i=1}^\obs \johnweights_{y, i} \projf_{y, i}^2 \cdot\sum_{i=1}^\obs \johnweights_{y, i} \projd_{y, i}^6 }^{1/2}
\end{align*}
Using the bound~\eqref{eq:john_exact_f_to_d_bound}, we obtain
\begin{align*}
\sum_{i=1}^\obs \johnweights_{y, i} \projf_{y, i}^2
\leq 4 \johnkappa^2 \sum_{i=1}^\obs \johnweights_{y, i} \projd_{y, i}^2
= 4 \johnkappa^2 \sum_{i=1}^\obs \johnweights_{x, i} \projd_{x, i}^2 \frac{\johnweights_{y, i}}{\johnweights_{x, i}} \frac{\projd_{y, i}^2}{\projd_{x, i}^2}.
% = 4 \frac{r^2}{\dims^{3/2} \johnkappa^2} \sum_{i=1}^\obs \johnweights_{x, i} \parenth{\hat{a}_{x, i}\tp \rvg}^2 \frac{\johnweights_{y, i}}{\johnweights_{x, i}} \frac{\projd_{y, i}^2}{\projd_{x, i}^2}
\end{align*}
Substituting $h = z-x$ where $z$ is given by relation~\eqref{eq:john_z_x_relation}, we obtain that \mbox{$\projd_{x, i} =  \frac{r}{\dims^{3/4}\johnkappa} \hat a_{x, i}\tp\rvg$},
% \begin{align}
%   \label{eq:john_d_to_rvg_relation}
%   \projd_{x, i} = a_i\tp h/\slack_{x, i} \defn \frac{r}{\dims^{3/4}\johnkappa^2} \hat a_{x, i}\tp\rvg
% \end{align}
and thereby
\begin{align*}
  \sum_{i=1}^\obs \johnweights_{y, i} \projf_{y, i}^2 \leq 4\johnkappa^2 \frac{r^2}{\dims^{3/2}\johnkappa^4} \sum_{i=1}^\obs \johnweights_{x, i} (\hat a_{x, i}\tp\rvg)^2 \frac{\johnweights_{y, i}}{\johnweights_{x, i}} \frac{\projd_{y, i}^2}{\projd_{x, i}^2}.
\end{align*}
Doing similar algebra, we obtain $\sum_{i=1}^\obs \johnweights_{y, i} \projd_{y, i}^6
 % = \sum_{i=1}^\obs \johnweights_{x, i} \projd_{x, i}^6 \frac{\johnweights_{y, i}}{\johnweights_{x, i}} \frac{\projd_{y, i}^6}{\projd_{x, i}^6}
 = \frac{r^6}{\dims^{9/2}\johnkappa^{12}} \sum_{i=1}^\obs \johnweights_{x, i} \parenth{\hat{a}_{x,i}\tp \rvg}^6 \frac{\johnweights_{y, i}}{\johnweights_{x, i}} \frac{\projd_{y, i}^6}{\projd_{x, i}^6}.$
Putting the pieces together yields the claim.
% paragraph bounding_ (end)

\paragraph{Bounding $C_3$:} % (fold)
\label{par:bounding_c_3}

Recall that $\projzsub_y = (\johnweightmatrix_y-\alpha \johnlaplacian_y)\projz_y$ (Lemma~\ref{lemma:john_gradient_and_hessian_and_bounds}) and $\johnftdinvmatrix_y = \parenth{\johnweightmatrix_y - \alpha \johnlaplacian_y}^{-1} \johnweightmatrix_y$ (Lemma~\ref{lemma:f_to_d_matrix}).
We have
\begin{align*}
  \abss{\sum_{i=1}^\obs \johnweights_{y, i} \projd_{y, i}^2 \projz_{y, i}}
  % = \mathbf{1}  \projdmatrix^2_y \johnweightmatrix_y \projzmatrix_y \mathbf{1}
  = \mathbf{1}  \projdmatrix^2_y \johnweightmatrix_y \projz_y
  = \underbrace{\mathbf{1}  \projdmatrix^2_y \johnweightmatrix_y (\johnweightmatrix_y-\alpha \johnlaplacian_y)^{-1}}_{=:\myvec_y\tp}\
   \underbrace{(\johnweightmatrix_y-\alpha \johnlaplacian_y)\projz_y}_{\projzsub_y}.
\end{align*}
Using the definition of $\myvec_y$ and $\johnftdinvmatrix_y$, we obtain
\begin{align*}
  \myvec_{y, i} \defn e_i\tp \myvec_y = e_i\tp\parenth{\johnweightmatrix_y - \alpha \johnlaplacian_y}^{-1} \johnweightmatrix_y \projdmatrix_y^2 \mathbf{1} = e_i\tp\johnftdinvmatrix_y \projdmatrix_y^2 \mathbf{1}
  = \johnftdinvmatrix_{y, i, i} \projd_{y, i}^2 + \sum_{j\in[\obs], j\neq i} \johnftdinvmatrix_{y, i, j} \projd_{y, j}^2.
\end{align*}
Consequently, we have
\begin{align*}
  \abss{\sum_{i=1}^\obs \myvec_{y, i} \projzsub_{y, i}}
  \leq
  \overbrace{\sum_{i=1}^\obs \abss{\projzsub_{y, i}} \cdot \abss{\johnftdinvmatrix_{y, i, i}\projd_{y, i}^2}}^{=:C_4}
  + \overbrace{\sum_{i=1}^\obs \abss{\projzsub_{y, i}} \cdot \parenth{
    \sum_{j\in[\obs], j\neq i} \abss{\johnftdinvmatrix_{y, i, j} \projd_{y, j}^2} }}^{=:C_5}
\end{align*}
From Lemma~\ref{lemma:f_to_d_matrix}, we have that $\johnftdinvmatrix_{y, i, i} \in [0, \johnkappa]$.
Hence, we have $C_4 \leq \vecnorm{\projzsub_y}{1} \cdot \johnkappa \cdot \max_{i \in [\obs]} \projd_{y, i}^2$.
To bound $C_5$, we note that
\begin{align*}
  \sum_{j\in[\obs], j\neq i} \abss{\johnftdinvmatrix_{y, i, j} \projd_{y, j}^2}
  \stackrel{(i)}{\leq} \parenth{\sum_{j\in[\obs], j\neq i}\frac{\johnftdinvmatrix_{y, i, j}^2}{\johnweights_{y, j}}
  \cdot \sum_{j=1}^\obs \johnweights_{y, j} \projd_{y, j}^4}^{1/2}
  \stackrel{(ii)}{\leq} \parenth{\johnkappa^3 \cdot \sum_{j=1}^\obs \johnweights_{x, j} \projd_{x, j}^4 \frac{\johnweights_{y, j}}{\johnweights_{x, j}} \frac{\projd_{y, j}^4}{\projd_{x, j}^4}}^{1/2},
\end{align*}
where step~$(i)$ follows from Cauchy-Schwarz inequality and step~$(ii)$ from Lemma~\ref{lemma:f_to_d_matrix}.
Putting the pieces together, we obtain that
\begin{align*}
      \abss{\sum_{i=1}^\obs \johnweights_{y, i} \projd_{y, i}^2 \projz_{y, i}}
      \leq \vecnorm{\projzsub_y}{1} \cdot \brackets{\johnkappa \cdot \max_{i \in [\obs]} \projd_{y, i}^2 + \johnkappa^{3/2} \parenth{\sum_{j=1}^\obs \johnweights_{x, j} \projd_{x, j}^4 \frac{\johnweights_{y, j}}{\johnweights_{x, j}} \frac{\projd_{y, j}^4}{\projd_{x, j}^4}}^{1/2}}.
\end{align*}
Using the bound on $\vecnorm{\projzsub_y}{1}$ from Lemma~\ref{lemma:john_gradient_and_hessian_and_bounds}, we have
\begin{align*}
  \abss{\sum_{i=1}^\obs \johnweights_{y, i} \projd_{y, i}^2 \projz_{y, i}}
  \leq \parenth{56 \johnkappa^2 \sum_{i=1}^\obs \johnweights_{y, i}\projd_{y, i}^2} \cdot
  \brackets{\johnkappa \cdot \max_{i \in [\obs]} \projd_{y, i}^2 + \johnkappa^{3/2} \parenth{\sum_{j=1}^\obs \johnweights_{x, j} \projd_{x, j}^4 \frac{\johnweights_{y, j}}{\johnweights_{x, j}} \frac{\projd_{y, j}^4}{\projd_{x, j}^4}}^{1/2}}.
\end{align*}
Substituting the expression for $\projd_{x, i}= \frac{r}{\johnkappa^2 \dims^{3/4}}\parenth{\hat{a}_{x,i}\tp \rvg}$ yields the claim.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Proofs of Lemmas from Section~\ref{sub:deterministic_bounds}} % (fold)
\label{sec:proofs_of_technical_lemmas_from_section_}

In this section we collect proofs of lemmas from Section~\ref{sub:deterministic_bounds}.
Each lemma is proved in a different subsection.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proof of Lemma~\ref{lemma:john_gradient_and_hessian_and_bounds}} % (fold)
\label{sub:proof_of_lemma_lemma:john_gradient_and_hessian_and_bounds}

\begin{subequations}
Up to second order terms, we have
\begin{align}
\frac{1}{\slack_{x+ h, i}^2} &= \frac{1}{\slack_{x,
    i}^2}\brackets{1+\frac{2a_i^\top h}{\slack_{x, i} } +
  \frac{3(a_i^\top h)^2}{\slack_{x, i}^2}  } + \order{\vecnorm{h}{2}^3},
\label{eq:john_expansion_of_s2}\\
    \johnweights_{y+h, i} &= \johnweights_{y, i} + h^\top \nabla \johnweights_{y, i} + \frac{1}{2} h^\top \nabla^2 \johnweights_{y, i} h + \order{\vecnorm{h}{2}^3}, \label{eq:john_expansion_of_g}\\
    \johnweights_{y+h, i}^\alpha &= \johnweights_{y, i}^\alpha + \alpha \johnweights_{y, i}^{\alpha-1}\parenth{h^\top \nabla \johnweights_{y, i}+\frac{1}{2} h^\top \nabla^2 \johnweights_{y, i} h} + \frac{\alpha\parenth{\alpha-1}}{2} \johnweights_{y, i}^{\alpha-2} \parenth{h^\top \nabla \johnweights_{y, i}}^2 + \order{\vecnorm{h}{2}^3}, \label{eq:john_expansion_of_g_alpha}
\end{align}
Further, let
\begin{align}
    \johnmod_y \defn A_y\tp \johnweightmatrix_y^\alpha A_y = \sum_{i=1}^\obs \johnweights_{y, i}^\alpha \frac{a_ia_i\tp}{\slack_{y, i}^2}.
    \label{eq:john_johnmod}
\end{align}
Using equations~\eqref{eq:john_expansion_of_s2} and \eqref{eq:john_expansion_of_g_alpha}, and substituting $\projd_{y, i} = a_i\tp h/\slack_{y, i}, \projf_{y, i} = h\tp \nabla \johnweights_{y, i}/\johnweights_{y, i}$ and $\projz_{y, i} = \frac{1}{2} h\tp \nabla^2 \johnweights_{y, i} h /\johnweights_{y, i}$, we find that
\begin{align*}
    \johnmod_{y+h}
    & = \sum_{i=1}^\obs \brackets{1 + \alpha \projf_{y, i} +
    \alpha \projz_{y, i} + \frac{\alpha\parenth{\alpha-1}}{2} \projf_{y, i}^2} \brackets{1+2\projd_{y, i}+3\projd_{y, i}^2 } \johnweights_{y, i}^\alpha \frac{a_ia_i^\top}{s_{y, i}^2}
    + \order{\vecnorm{h}{2}^3}.
\end{align*}
Note that $\projd_{y, i}$ and $\projf_{y, i}$ are first order terms in $\vecnorm{h}{2}$ and $\projz_{y, i}$ is a second order term in $\vecnorm{h}{2}$.

Thus we obtain
\begin{align*}
    \johnmod_{y+h} - \johnmod_y &= \underbrace{\sum_{i=1}^\obs \parenth{ 2 \projd_{y, i} + \alpha \projf_{y, i} } \johnweights_{y, i}^\alpha \frac{a_ia_i^\top}{s_{y, i}^2}}_{=:\Delta_{y, h}^{(1)}}\\
     &+  \underbrace{\sum_{i=1}^\obs \brackets{3\projd_{y, i}^2 + 2 \alpha \projd_{y, i} \projf_{y, i} + \alpha \projz_{y, i}  + \frac{\alpha(\alpha-1)}{2} \projf_{y, i}^2 }\johnweights_{y, i}^\alpha \frac{a_ia_i^\top}{s_{y, i}^2}}_{=:\Delta_{y, h}^{(2)}} + \order{\vecnorm{h}{2}^3}.
    % & = \Delta_{y, 1} + \Delta_{y, 2},
\end{align*}
Let $\Delta_{y, h}  \defn \Delta_{y, h}^{(1)} + \Delta_{y, h}^{(2)}$.
Note that $\Delta_{y, h}^{(i)}$ denotes the $i$-th order term in $\vecnorm{h}{2}$.
Finally, the following expansion also comes in handy for our derivations:
\begin{align}
a_i^T \johnmod_{y+ h}^{-1} a_i &= a_i^\top \johnmod_y^{-1}a_i -
a_i^\top \johnmod_y^{-1} \Delta_{y, h} \johnmod_y^{-1} a_i
+ a_i^\top \johnmod_y^{-1} \Delta_{y, h} \johnmod_y^{-1}
\Delta_{y, h} \johnmod_y^{-1} a_i
+ \order{\vecnorm{h}{2}^3}.
\label{eq:john_expansion_of_johnmod}
\end{align}
\end{subequations}
\subsubsection{Proof of part~\ref{item:gradient_g}: Gradient of weights} % (fold)
\label{ssub:proof_of_part_item:gradient_g}
The expression for the gradient $\nabla \johnweights_{y, i}$ is derived in Lemma~14 of the paper~\citep{lee2014path} and is thereby omitted.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Proof of part~\ref{item:hessian_g}: Hessian of weights} % (fold)
\label{ssub:proof_of_part_item:hessian_g}
We claim that
\begin{align}
    \projzsub_{y} = \parenth{\Ind - \alpha \johnlaplacian_y \johnweightmatrix_y^{-1}}
    \begin{bmatrix}
        \frac{1}{2} h^\top \nabla^2 \johnweights_{y, 1} h \\ \cdots \\ \frac{1}{2} h^\top \nabla^2 \johnweights_{y, m} h
    \end{bmatrix}
    & = (2 \projdmatrix_y + \alpha \projfmatrix_y) \johnprojmatrix_y^{(2)}  (2 \projdmatrix_y + \alpha \projfmatrix_y) \mathbf{1} \nonumber \\
    & + \parenth{\johnlevmatrix_y - \johnprojmatrix_y^{(2)}} \brackets{2 \alpha \projdmatrix_y\projfmatrix_y + 3 \projdmatrix_y^2 + \alphaprod \projfmatrix_y^2 } \mathbf{1} \nonumber \\
    & + \diag \parenth{ \johnprojmatrix_y (2\projdmatrix_y + \alpha \projfmatrix_y)   \johnprojmatrix_y (2\projdmatrix_y + \alpha \projfmatrix_y) \johnprojmatrix_y },
\label{eq:john_hessians_of_g}
\end{align}
where we have used $\diag(\mymat)$ to denote the diagonal vector $(\mymat_{1, 1}, \ldots, \mymat_{\obs, \obs})$ of the matrix $\mymat$.
Deferring the proof of this expression for the moment, we now derive a bound on the $\ell_1$ norm of $\projzsub_y$.
Expanding the $i$-th term of $\projzsub_{y, i}$ from equation~\eqref{eq:john_hessians_of_g}, we obtain
 \begin{align*}
    \projzsub_{y, i} &= (2\projd_{y, i} + \alpha \projf_{y, i} ) \sum_{j=1}^\obs (2 \projd_{y, j} + \alpha \projf_{y, j}) \johnprojmatrix_{y, i, j}^2
   + \brackets{2 \alpha \projd_{y, i} \projf_{y, i} +  3\projd_{y, i}^2 +
   \alphaprod \projf_{y, i}^2} \levjohn_{y, i} \\
   &\quad - \sum_{j=1}^\obs \brackets{2 \alpha \projd_{y, j} \projf_{y, j} + 3\projd_{y, j}^2 + \alphaprod \projf_{y, j}^2 } \johnprojmatrix_{y, i, j}^2
   + \sum_{j, l=1}^\obs (2 \projd_{y, j} + \alpha \projf_{y, j}) (2 \projd_{y, l}  + \alpha \projf_{y, l} ) \johnprojmatrix_{y, i, j} \johnprojmatrix_{y, j, l} \johnprojmatrix_{y, l, i}.
  \end{align*}
  Recall that $\alpha = 1-1/\log_2(2\obs/\dims)$.
  Since $\obs \geq \dims$ for polytopes, we have $\alpha \in [0, 1]$ and consequently $\vert \alphaprod \vert = \vert \alpha (\alpha-1)/2\vert \in [0, 1]$.
  Further note that $\johnprojmatrix_x$ is an orthogonal projection matrix, and hence we have
\begin{align*}
  \diag(\johnprojmatrix_x e_i) \johnprojmatrix_x \diag(\johnprojmatrix_x e_i)
  \preceq \diag(\johnprojmatrix_x e_i)\diag(\johnprojmatrix_x e_i).
\end{align*}
  Combining these observations with the AM-GM inequality, we have
  \begin{align*}
  \abss{\projzsub_{y, i}}
  &\leq 7 \levjohn_{y, i} \projd_{y, i}^2 + 3 \levjohn_{y, i} \projf_{y, i}^2 + \sum_{j=1}^\obs \parenth{ 13\projd_{y, j}^2 + 6 \projf_{y, j}^2} \johnprojmatrix_{y, i, j}^2.
\end{align*}
Summing both sides over the index $i$, we find that
\begin{align*}
\sum_{i=1}^\obs  \abss{\projzsub_{y, i}}
\stackrel{(i)}{\leq} \sum_{i=1}^\obs 20 \levjohn_{y, i} \projd_{y, i}^2 + 9 \levjohn_{y, i} \projf_{y, i}^2
\stackrel{(ii)}{\leq} \sum_{i=1}^\obs 20 \johnweights_{y, i} \projd_{y, i}^2 + 9 \johnweights_{y, i} \projf_{y, i}^2
\stackrel{(iii)}{\leq} 56\johnkappa^2 \sum_{i=1}^\obs \johnweights_{y, i} \projd_{y, i}^2,
\end{align*}
where step $(i)$ follows from Lemma~\ref{ppt:john_all_properties}~\ref{item:john_sigma_properties}, step $(ii)$ from Lemma~\ref{lemma:john_first_bounds}~\ref{item:john_weight_equality} and step $(iii)$ from the bound~\eqref{eq:john_exact_f_to_d_bound}.


We now return to the proof of expression~\eqref{eq:john_hessians_of_g}.
Using equation~\eqref{eq:john_normal_equation}, we find that
\begin{align}
    \frac{1}{2} h\tp \nabla^2 \johnweights_{y, i} h = \frac{1}{2} h \tp \nabla^2 \levjohn_{y, i} h \quad \text{ for all } i \in [\obs].
    \label{eq:john_equality_of_hessians}
\end{align}
Next, we derive the Taylor series expansion of $\levjohn_{y, i}$.
Using the definition of $\johnmod_x$~\eqref{eq:john_johnmod} in equation~\eqref{eq:john_projection_matrix}, we find that $\levjohn_{y, i} = \johnweights_{y, i}^\alpha\frac{a_i\tp \johnmod_{y}^{-1}a_i}{\slack_{y, i}^2}$.
To compute the difference $\levjohn_{y+h, i} - \levjohn_{y, i}$, we use the expansions~\eqref{eq:john_expansion_of_s2}, \eqref{eq:john_expansion_of_g_alpha} and \eqref{eq:john_expansion_of_johnmod}.
Letting $\alphaprod = \alpha(\alpha-1)/2$, we have
\begin{align*}
    \levjohn_{y+h, i}
    & = \johnweights_{y+h, i}^\alpha \frac{a_i^\top \johnmod_{y+h}^{-1} a_i}{\slack_{y+h,i}^2}\\
    & = \johnweights_{y, i}^\alpha \frac{a_i^\top \johnmod_{y+h}^{-1} a_i}{\slack_{y,i}^2} \brackets{1 + \alpha \projf_{y, i}
        +\alpha \projz_{y, i}
        +\alphaprod \projf_{y, i}^2} \brackets{1+2\projd_{y, i} + 3\projd_{y, i}^2} + \order{\vecnorm{h}{2}^3}\\
    & = \levjohn_{y, i} + (2\projd_{y, i} + \alpha \projf_{y, i}) \levjohn_{y, i} - \sum_{j=1}^\obs (2 \projd_{y, j} + \alpha \projf_{y, j}) \johnprojmatrix_{y, i, j}^2 + (2\projd_{y, i} + \alpha \projf_{y, i} ) \sum_{j=1}^\obs (2 \projd_{y, j} + \alpha \projf_{y, j}) \johnprojmatrix_{y, i, j}^2 \\
    & \quad + 2 \alpha \projd_{y, i} \projf_{y, i} \levjohn_{y, i} + \brackets{\alpha \projz_{y, i}+ \alphaprod \projf_{y, i}^2 + 3\projd_{y, i}^2} \levjohn_{y, i}
    - \sum_{j=1}^\obs \brackets{3\projd_{y, j}^2 + 2 \alpha \projd_{y, j} \projf_{y, j} + \alpha \projz_{y, j} + \alphaprod \projf_{y, j}^2 } \johnprojmatrix_{y, i, j}^2 \\
    & \quad + \sum_{j, l=1}^\obs (2 \projd_{y, j} + \alpha \projf_{y, j}) (2 \projd_{y, l}  + \alpha \projf_{y, l} ) \johnprojmatrix_{y, i, j} \johnprojmatrix_{y, j, l} \johnprojmatrix_{y, l, i} + \order{\vecnorm{h}{2}^3}.
\end{align*}
We identify the second order (in \order{\vecnorm{h}{2}^2}) terms in the previous expression.
Using the equation~\eqref{eq:john_equality_of_hessians}, these are indeed the terms that correspond to the terms $\frac{1}{2} h^\top \nabla^2 \johnweights_{y, i} h$, $i \in [\obs]$.
Substituting $\projz_{y, i} = \frac{1}{2}h\tp \nabla^2 \johnweights_{y, i} h / \johnweights_{y, i}$, we have
\begin{align*}
    &\frac{1}{2} h^\top \nabla^2 \johnweights_{y, i} h \\
    &= (2\projd_{y, i} + \alpha \projf_{y, i} ) \sum_{j=1}^\obs (2 \projd_{y, j} + \alpha \projf_{y, j}) \johnprojmatrix_{y, i, j}^2 + 2 \alpha \projd_{y, i} \projf_{y, i} \levjohn_{y, i}
    + \brackets{\frac{\alpha}{2} \frac{h^\top \nabla^2 \johnweights_{y, i} h}{\johnweights_{y,i}} + \alphaprod \projf_{y, i}^2 + 3\projd_{y, i}^2} \levjohn_{y, i} \\
    & - \sum_{j=1}^\obs \brackets{3\projd_{y, j}^2 + 2 \alpha \projd_{y, j} \projf_{y, j} + \frac{\alpha}{2} \frac{h^\top \nabla^2 \johnweights_{y, j} h}{\johnweights_{y,j}} + \alphaprod \projf_{y, j}^2 } \johnprojmatrix_{y, i, j}^2
    + \sum_{j, l=1}^\obs (2 \projd_{y, j} + \alpha \projf_{y, j}) (2 \projd_{y, l}  + \alpha \projf_{y, l} ) \johnprojmatrix_{y, i, j} \johnprojmatrix_{y, j, l} \johnprojmatrix_{y, l, i}.
\end{align*}

Collecting the different terms and doing some algebra yields the result~\eqref{eq:john_hessians_of_g}.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Proof of part~\ref{item:gradient_log_det}: Gradient of logdet} % (fold)
\label{ssub:proof_of_part_item:gradient_log_det}
For a unit vector $h \in \realdim$, we have
\begin{align*}
    h\tp \log\det J_y &= \lim_{\delta \rightarrow 0}\frac{1}{\delta}(\log\det J_{y+ \delta h} - \log\det J_y)
    = \lim_{\delta \rightarrow 0}\frac{1}{\delta}(\log\det J_y^{-1/2}J_{y+ \delta h}J_y^{-1/2} - \log\det \Ind_\dims)
\end{align*}
Let $\hat a_{y, i} \defn \john_{y, i}^{-1/2}a_i/\slack_{y, i}$ for each $i \in [\obs]$.
Using the property $\log \det B = \trace\log B$, where $\log B$ denotes the logarithm of the matrix and that $\log \det \Ind_\dims = 0$,
% the facts that $\sum_{i=1}^\obs \johnweights_{y, i} \hat a_{y, i} \hat a_{y, i}\tp = \Ind_\dims$,
we obtain
\begin{align*}
    h\tp \log\det J_y = \lim_{\delta \rightarrow 0} \frac{1}{\delta} \brackets{ \trace\log \parenth{\sum_{i=1}^\obs \frac{\johnweights_{y+\delta h}}{(1-\delta a_i\tp h/\slack_{y, i})} \hat a_{y, i} \hat a_{y, i}\tp} },
\end{align*}
where we have substituted $\slack_{y+\delta h, i} = \slack_{y, i} - \delta a_i\tp h$.
Keeping track of first order terms in $\delta$, and noting that $\sum_{i=1}^\obs \johnweights_{y, i} \hat a_{y, i} \hat a_{y, i}\tp = \Ind_\dims$, we find that
\begin{align*}
    \trace\log \parenth{\sum_{i=1}^\obs \frac{\johnweights_{y+\delta h, i}}{(1-\delta a_i\tp h/\slack_{y, i})} \hat a_{y, i} \hat a_{y, i}\tp}
    &= \trace\log \brackets{\sum_{i=1}^\obs \parenth{\johnweights_{y, i} + \delta h\tp \nabla \johnweights_{y, i} } \parenth{1+\frac{2\delta a_i\tp h}{\slack_{y, i}}} \hat a_{y, i} \hat a_{y, i}\tp} + \order{\delta^2}\\
    & = \trace \brackets{\sum_{i=1}^\obs \delta \parenth{\frac{2a_i\tp h}{\slack_{y, i}} + h\tp \nabla \johnweights_{y, i}} \hat a_{y, i} \hat a_{y, i}\tp} + \order{\delta^2}\\
    & = \sum_{i=1}^\obs \delta \parenth{\frac{2a_i\tp h}{\slack_{y, i}} + h\tp \nabla \johnweights_{y, i}} \johnlocalslack_{y, i} + \order{\delta^2}
\end{align*}
where in the last step we have used the fact that $\trace(\hat a_{y, i} \hat a_{y, i}\tp) = \hat a_{y, i} \tp \hat a_{y, i} = \johnlocalslack_{y, i}$ for each $i \in [\obs]$.
Substituting the expression for $\nabla \johnweights_{y}$ from part~\ref{item:gradient_g}, and rearranging the terms yields the claimed expression in the limit $\delta \rightarrow 0$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Proof of part~\ref{item:gradient_phi}: Gradient of $\johnphi$} % (fold)
\label{ssub:proof_of_part_item:gradient_phi}
Using the chain rule and the fact that $\nabla \slack_{y, i} = -a_i$, yields the result.
\subsubsection{Proof of part~\ref{item:john_hessian_log_det_bound}} % (fold)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{ssub:proof_of_part_ref}
We claim that
\begin{align*}
      \frac{1}{2} h \tp \hesslogdetJ_y h
      = \frac{1}{2}\brackets{\sum_{i=1}^\obs \johnweights_{y, i} \johnlocalslack_{y, i} (3\projd_{y, i}^2 + 2 \projd_{y, i}\projf_{y, i} + \projz_{y, i}) - \frac{1}{2} \sum_{i, j=1}^\obs \johnweights_{y, i} \johnweights_{y, j} \johnlocalslack_{y, i, j}^2 \parenth{2\projd_{y, i} + \projf_{y, i}} \parenth{2\projd_{y, j} + \projf_{y, j}}}.
    \end{align*}
The desired bound on $\abss{h \tp \hesslogdetJ_y h}/2$ now follows from an application of AM-GM inequality with Lemma~\ref{ppt:john_all_properties}\ref{item:john_theta_properties}.

We now derive the claimed expression for the directional Hessian of the function $\logdetJ$.
We have
\begin{align*}
    &\frac{1}{2} h\tp \parenth{\nabla^2 \log\det J_y} h
    = \lim_{\delta \rightarrow 0}\frac{1}{2\delta^2}(\log\det J_y^{-1/2}J_{y+ \delta h}J_y^{-1/2} + \log\det J_y^{-1/2}J_{y- \delta h}J_y^{-1/2} - 2\log\det \Ind_\dims)  \\
    &= \frac{1}{2} \lim_{\delta \rightarrow 0} \frac{1}{\delta^2} \brackets{ \trace\log \parenth{\sum_{i=1}^\obs \frac{\johnweights_{y+\delta h}}{(1-\delta a_i\tp h/\slack_{y, i})} \hat a_{y, i} \hat a_{y, i}\tp} +
    \trace\log \parenth{\sum_{i=1}^\obs \frac{\johnweights_{y-\delta h}}{(1+\delta a_i\tp h/\slack_{y, i})} \hat a_{y, i} \hat a_{y, i}\tp} }.
\end{align*}
\noindent Expanding the first term in the above expression, we find that
\begin{align*}
    &\trace\log \parenth{\sum_{i=1}^\obs \frac{\johnweights_{y+\delta h, i}}{(1-\delta a_i\tp h/\slack_{y, i})} \hat a_{y, i} \hat a_{y, i}\tp}\\
    &= \trace\log \underbrace{\brackets{
    \sum_{i=1}^\obs
    \parenth{\johnweights_{y, i} + \delta h\tp \nabla \johnweights_{y, i} + \frac{\delta^2}{2} h\tp \nabla^2 \johnweights_{y, i} h }
    \parenth{1+2\delta\frac{a_i\tp h}{\slack_{y, i}} + 3\delta^2\frac{(a_i\tp h)^2}{\slack_{y, i}^2}}
    \hat a_{y, i} \hat a_{y, i}\tp
     }}_{=:\Ind_\dims + \mymat}
     + \order{\delta^3}.
    % &= \trace \Bigg[
    % \sum_{i=1}^\obs
    % \johnweights_{y, i}
    % \parenth{2\delta\frac{a_i\tp h}{\slack_{y, i}} + 3\delta^2\frac{(a_i\tp h)^2}{\slack_{y, i}^2}}
    % \hat a_{y, i} \hat a_{y, i}\tp
    %  \Bigg]
    %  \\
    %  &\quad + \trace \Bigg[
    % \sum_{i=1}^\obs
    % \parenth{\delta h\tp \nabla \johnweights_{y, i} + \frac{\delta^2}{2} h\tp \nabla^2 \johnweights_{y, i} h }
    % \parenth{1 + 2\delta\frac{a_i\tp h}{\slack_{y, i}} + 3\delta^2\frac{(a_i\tp h)^2}{\slack_{y, i}^2}}
    % \hat a_{y, i} \hat a_{y, i}\tp
    %  \Bigg]\\
    %  &\quad - \frac{1}{2} \trace \brackets{
    % \sum_{i=1}^\obs
    % \parenth{\johnweights_{y, i} + \delta h\tp \nabla \johnweights_{y, i} + \frac{\delta^2}{2} h\tp \nabla^2 \johnweights_{y, i} h }
    % \parenth{2\delta\frac{a_i\tp h}{\slack_{y, i}} + 3\delta^2\frac{(a_i\tp h)^2}{\slack_{y, i}^2}}
    % \hat a_{y, i} \hat a_{y, i}\tp
    %  }^2
    %  +  \order{\delta^3},\\
    %  & = \sum_{i=1}^\obs \johnlocalslack_{y, i} \johnweights_{y, i} \parenth{1 + \delta \projf_{y, i} + \delta^2 \projz_{y, i}} \parenth{2\delta \projd_{y, i} + 3\delta^2 \projd_{y, i}^2}\\
    %  &\quad -\frac{1}{2} \sum_{i, j=1}^\obs \johnlocalslack_{y, i, j}^2\johnweights_{y, i} \johnweights_{y, j}  \parenth{1 + \delta \projf_{y, i} + \delta^2 \projz_{y, i}} \parenth{2\delta \projd_{y, i} + 3\delta^2 \projd_{y, i}^2}  \parenth{1 + \delta \projf_{y, j} + \delta^2 \projz_{y, j}} \parenth{2\delta \projd_{y, j} + 3\delta^2 \projd_{y, j}^2}
\end{align*}
Substituting the shorthand notation from equations~\eqref{eq:john_def_D}, \eqref{eq:john_def_F} and \eqref{eq:john_def_Z}, we have
\begin{align*}
    \mymat
    % &= \sum_{i=1}^\obs \johnweights_{y, i} \parenth{2\delta \projd_{y, i}  +3 \delta^2 \projd_{y, i}^2 + \parenth{\delta \projf_{y, i} + \delta^2 \projz_{y, i}} \parenth{1+2\delta\projd_{y, i} + 3\delta^2 \projd_{y, i}}} \hat a_{y, i} \hat a_{y, i}\tp\\
    &=\sum_{i=1}^\obs \johnweights_{y, i} \brackets{\delta (2\projd_{y, i} + \projf_{y, i})
    + \delta^2 (3\projd_{y, i}^2 + 2 \projd_{y, i}\projf_{y, i} + \projz_{y, i})} \hat a_{y, i} \hat a_{y, i}\tp + \order{\delta^3}.
\end{align*}
Now we make use of the following facts (1) $\trace\log (\Ind_\dims + \mymat) = \trace\brackets{\mymat - \frac{\mymat^2}{2} + \order{\vecnorm{\mymat}{}^3}}$, (2) for each $i, j \in [\obs]$, we have $\trace(\hat a_{y, i} \hat a_j\tp) = \hat a_{y, i} \tp \hat a_j = \johnlocalslack_{y, i, j}$, and (3) for each $i \in [\obs]$, we have $\johnlocalslack_{y, i, i} = \johnlocalslack_{y, i}$.
Thus we obtain
\begin{align*}
    \trace\log \parenth{\sum_{i=1}^\obs \frac{\johnweights_{y+\delta h, i}}{(1-\delta a_i\tp h/\slack_{y, i})} \hat a_{y, i} \hat a_{y, i}\tp}
    &= \sum_{i=1}^\obs \johnweights_{y, i} \johnlocalslack_{y, i} \brackets{\delta (2\projd_{y, i} + \projf_{y, i})
    + \delta^2 (3\projd_{y, i}^2 + 2 \projd_{y, i}\projf_{y, i} + \projz_{y, i})} \\
    &\quad - \frac{1}{2} \sum_{i, j=1}^\obs \johnweights_{y, i} \johnweights_{y, j} \johnlocalslack_{y, i, j}^2 \delta^2 (2\projd_{y, i} + \projf_{y, i})   (2\projd_{y, j} + \projf_{y, j})
    + \order{\delta^3}.
\end{align*}
Similarly, we can obtain an expression for $\trace\log \parenth{\sum_{i=1}^\obs \frac{\johnweights_{y-\delta h}}{(1+\delta a_i\tp h/\slack_{y, i})} \hat a_{y, i} \hat a_{y, i}\tp}$.
Putting the pieces together, we obtain
\begin{align}
    \frac{1}{2} h\tp \parenth{\nabla^2 \log\det J_y} h = \sum_{i=1}^\obs \johnweights_{y, i} \johnlocalslack_{y, i} (3\projd_{y, i}^2 + 2 \projd_{y, i}\projf_{y, i} + \projz_{y, i})
    - \frac{1}{2} \sum_{i, j=1}^\obs \johnweights_{y, i} \johnweights_{y, j} \johnlocalslack_{y, i, j}^2 (2\projd_{y, i} + \projf_{y, i})   (2\projd_{y, j} + \projf_{y, j}).
    \label{eq:john_final_hess_detj_expression}
\end{align}
% \begin{align*}
%     \frac{1}{2} h\tp \hesslogdetJ_y h
%     &\leq
%     \sum_{i=1}^\obs \johnweights_{y, i} \johnlocalslack_{y, i} (4\projd_{y, i}^2 + \projf_{y, i}^2 + \projz_{y, i})
%     + \frac{1}{2} \sum_{i, j=1}^\obs \johnweights_{y, i} \johnweights_{y, j} \johnlocalslack_{y, i, j}^2 (3\projd_{y, i}^2 + 3\projd_{y, j}^2 + \frac{3}{2}\projf_{y, i}^2 + \frac{3}{2}\projf_{y, j}^2)\\
%     &=\sum_{i=1}^\obs \johnweights_{y, i} \johnlocalslack_{y, i} (7\projd_{y, i}^2 + \frac{5}{2}\projf_{y, i}^2 + \projz_{y, i}),
% \end{align*}
% where in the last step we have applied Lemma~\ref{ppt:john_all_properties}\ref{item:john_theta_properties}.
% subsection proof_of_part_ref (end)


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Proof of part~\ref{item:hessian_beta_bound}} % (fold)
\label{ssub:proof_of_part_item:hessian_beta_bound}
We claim that
\begin{align}
\frac{1}{2} h\tp \nabla^2 \johnphi_{y, i} h = \johnphi_{y, i} \parenth{2 \projd_{y, i} \projf_{y, i} + 3 \projd_{y, i}^2 + \projz_{y, i}}.
\label{eq:john_hessian_phi}
\end{align}
The claim follows from a straightforward application of chain rule and substitution of the expressions for $\nabla \johnweights_{y, i}$ and $\nabla^2 \johnweights_{y, i}$ in terms of the shorthand notation $\projd_{y, i}, \projf_{y, i}$ and $\projz_{y, i}$.
Multiplying both sides of equation~\eqref{eq:john_hessian_phi} with $\projd_{y, i}^2\slack_{y, i}^2$ and summing over index $i$, we find that
\begin{align*}
    \sum_{i=1}^\obs \projd_{y, i}^2 \slack_{y, i}^2 \frac{1}{2} h\tp \nabla \johnphi_{y, i}^2 h
    = \sum_{i=1}^\obs \projd_{y, i}^2 \slack_{y, i}^2 \johnphi_{y, i}\brackets{\projz_{y, i} + 2\projd_{y, i} \projf_{y, i} + 3 \projd_{y, i}^2}
    &= \sum_{i=1}^\obs \projd_{y, i}^2 \johnweights_{y, i}\brackets{\projz_{y, i} + 2\projd_{y, i} \projf_{y, i} + 3 \projd_{y, i}^2}\\
    &\leq\sum_{i=1}^\obs \projd_{y, i}^2 \johnweights_{y, i}\brackets{\projz_{y, i} + \projf_{y, i}^2 + 4 \projd_{y, i}^2},
\end{align*}
where in the last step we have used the AM-GM inequality.
The claim follows.

%% JOHN Lemmas

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Lemma~\ref{lemma:f_to_d_l2}} % (fold)
\label{sub:proof_of_lemma_lemma:f_to_d_l2}

% \begin{proof}[Proof of Lemma~\ref{lemma:f_to_d_l2}]
  We claim that
  \begin{align}
    \label{eq:john_f_to_d_intermediate}
    0 \preceq \johnweightmatrix_y^{-1/2} \parenth{c_1 \Ind_\obs + c_2 \johnlaplacian_y \parenth{\johnweightmatrix_y-\alpha\johnlaplacian_y}^{-1}} \johnweightmatrix_y^{1/2} \preceq \parenth{c_1 + c_2}\johnkappa \Ind_\obs.
  \end{align}
  The proof of the lemma is immediate from this claim, as for any PSD matrix $H \leq c\Ind_\obs$, we have $H^2 \leq c^2 \Ind_\obs$.

  We now prove claim~\eqref{eq:john_f_to_d_intermediate}.
  Note that
  \begin{align}
     \johnweightmatrix_y^{-1/2}\johnlaplacian_y \parenth{\johnweightmatrix_y-\alpha\johnlaplacian_y}^{-1} \johnweightmatrix_y^{1/2}
     = \underbrace{\johnweightmatrix_y^{-1/2}\johnlaplacian_y \johnweightmatrix_y^{-1/2}}_{:=\mymat_y}
     (\Ind_\obs -\johnalpha \johnweightmatrix_y^{-1/2}\johnlaplacian_y \johnweightmatrix_y^{-1/2})^{-1}.
     \label{eq:john_equality_glg}
  \end{align}
  Note that the RHS is equal to the matrix $\mymat_y (\Ind_\obs - \alpha_\tagjohn \mymat_y)^{-1}$ which is symmetric.
  Observe the following ordering of the matrices in the PSD cone
  \begin{align*}
    \johnlevmatrix_y + \johnbeta \Ind_\obs = \johnweightmatrix_y
    \succeq \johnlevmatrix_y
    \succeq \johnlaplacian_y = \johnlevmatrix_y - \johnprojmatrix_y^{(2)}
    \succeq 0.
  \end{align*}
  For the last step we have used the fact that $ \johnlevmatrix_y - \johnprojmatrix_y^{(2)}$ is a diagonally dominant matrix with non negative entries on the diagonal to conclude that it is a PSD matrix.
  Consequently, we have
  \begin{align}
  \label{eq:john_glg}
    \mymat_y = \johnweightmatrix_y^{-1/2}\johnlaplacian_y \johnweightmatrix_y^{-1/2} \preceq \Ind_\obs.
  \end{align}
  Further, recall that $\johnalpha = (1-1/\johnkappa) \Leftrightarrow \johnkappa = (1-\johnalpha)^{-1}$.
  As s result, we obtain
  \begin{align*}
    0 \preceq (\Ind_\obs-\johnalpha\johnweightmatrix_y^{-1/2}\johnlaplacian_y \johnweightmatrix_y^{-1/2} )^{-1} \preceq \johnkappa \Ind_\obs.
  \end{align*}
  Multiplying both sides by $\mymat_y^{1/2}$ and using the relation~\eqref{eq:john_glg}, we obtain
  \begin{align}
    0 \preceq \mymat_y^{1/2}  (\Ind_\obs-\johnalpha\johnweightmatrix_y^{-1/2}\johnlaplacian_y \johnweightmatrix_y^{-1/2} )^{-1} \mymat_y^{1/2} \preceq \johnkappa \Ind_\obs.
    \label{eq:john_G_laplace_G_bound}
  \end{align}
  Using the fact that $\mymat_y$ commutes with $(\Ind_\obs - \mymat_y)^{-1}$, we obtain $\mymat_y (\Ind_\obs-\johnalpha\mymat_y)^{-1} \preceq \johnkappa \Ind_\obs$.
  Using observation~\eqref{eq:john_equality_glg} now completes the proof.
% \end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proof of Lemma~\ref{lemma:f_to_d_matrix}} % (fold)
\label{sub:proof_of_lemma_lemma:f_to_d_matrix}

% \begin{proof}[Proof of Lemma~\ref{lemma:f_to_d_matrix}]

Without loss of generality, we can first prove the result for $i=1$.
Let $\johnftdinvvector \defn \johnftdinvmatrix_y\tp e_1$ denote the first row of the matrix $\johnftdinvmatrix_y$.
Observe that
\begin{align}
    \label{eq:john_F_to_D_infinity_bound}
    e_1
    = \parenth{\johnweightmatrix_y - \alpha \johnlaplacian_y} \johnweightmatrix_y^{-1} \johnftdinvvector
    = \johnftdinvvector - \alpha \johnlevmatrix_y \johnweightmatrix_y^{-1} \johnftdinvvector + \alpha \johnprojmatrix_y^{(2)} \johnweightmatrix_y^{-1} \johnftdinvvector
    % \nonumber
\end{align}
We now prove bounds~\eqref{eq:john_mu_first_coordinate_bound} and \eqref{eq:john_mu_sum_of_terms_bound} separately.

% We proceed with our analysis in two steps: (1) First, we isolate $\johnftdinvvector_1$ (the first coordinate of $\johnftdinvvector$) and establish an upper and lower bound for $\johnftdinvvector_1$, and (2) second, we obtain a weighted $\ell_2$-norm bound on the vector $\tilde\johnftdinvvector = (\johnftdinvvector_2, \ldots, \johnftdinvvector_\obs)\tp$.

\paragraph{Proof of bound~\eqref{eq:john_mu_first_coordinate_bound}:} % (fold)
\label{par:proof_of_bound_eq:john_mu_first_coordinate_bound}

% \paragraph*{Step (1):} % (fold)
% \label{par:step_1_}
Multiplying the equation~\eqref{eq:john_F_to_D_infinity_bound} on the left by $\johnftdinvvector \tp \johnweightmatrix_y^{-1}$, we obtain
\begin{align}
  g_1^{-1} \johnftdinvvector_1
  &= \johnftdinvvector \tp \johnweightmatrix_y^{-1} \johnftdinvvector - \alpha \johnftdinvvector \tp \johnweightmatrix_y^{-1} \johnlevmatrix_y \johnweightmatrix_y^{-1} \johnftdinvvector + \alpha \johnftdinvvector \tp \johnweightmatrix_y^{-1} \johnprojmatrix_y^{(2)} \johnweightmatrix_y^{-1} \johnftdinvvector \notag \\
  & \geq \johnftdinvvector \tp \johnweightmatrix_y^{-1} \johnftdinvvector - \alpha \johnftdinvvector \tp \johnweightmatrix_y^{-1} \johnlevmatrix_y \johnweightmatrix_y^{-1} \johnftdinvvector
  \label{eq:john_F_to_D_infinity_bound_upper}
  \\
  & \geq \parenth{g_1^{-1} - \alpha \levjohn_{y, 1}/g_1^2} \johnftdinvvector_1^2. \notag
\end{align}
Rearranging terms, we obtain
\begin{align}
0 \leq \johnftdinvvector_1 \leq \frac{\johnweights_{y, 1}}{\johnweights_{y, 1} -\alpha \levjohn_{y, 1}} \stackrel{(i)}{\leq} \johnkappa,
\label{eq:john_upper_bound_mu1}
\end{align}
where  inequality (i) follows from the facts that $\johnweights_{y, j} \geq \levjohn_{y, j}$ and  $(1-\alpha) = \johnkappa$.

% Thus we have established the claimed bounds.
% paragraph proof_of_bound_eq:john_mu_first_coordinate_bound (end)

\paragraph{Proof of bound~\eqref{eq:john_mu_sum_of_terms_bound}:} % (fold)
\label{par:proof_of_bound_eq:john_mu_sum_of_terms_bound}
In our proof, we  use the following improved lower bound for the term $\johnftdinvmatrix_{y, 1, 1} = \johnftdinvvector_1$.
\begin{align}
\johnftdinvvector_1 \geq \frac{\johnweights_{y, 1}}{\johnweights_{y, 1} - \alpha \levjohn_{y, 1} + \alpha \levjohn_{y, 1}^2},
\label{eq:john_lower_bound_mu1}
\end{align}
Deferring the proof of this claim at the moment, we now complete the proof.

We begin by deriving a weighted $\ell_2$-norm bound for the vector $\tilde\johnftdinvvector = (\johnftdinvvector_2, \ldots, \johnftdinvvector_\obs)\tp$.
Equation~\eqref{eq:john_F_to_D_infinity_bound_upper} implies
\begin{align*}
\johnweights_{y, 1}^{-1} \johnftdinvvector_1 \parenth{1- \johnftdinvvector_1 + \alpha \frac{\levjohn_{y, 1}}{\johnweights_{y, 1}} \johnftdinvvector_1 } \geq \sum_{j=2}^\obs \johnftdinvvector_j^2 \parenth{\johnweights_{y, j}^{-1} - \alpha \johnweights_{y, j}^{-2} \levjohn_{y, j}}
\stackrel{(i)}{\geq} (1-\alpha)
\sum_{j=2}^\obs \frac{\johnftdinvvector_j^2}{\johnweights_{y, j}},
\end{align*}
where step $(i)$ follows from the fact that $\johnweights_{y, i} \geq \levjohn_{y, i}$.
Now, we upper bound the expression on the left hand side of the above inequality using the upper~\eqref{eq:john_upper_bound_mu1} and lower~\eqref{eq:john_lower_bound_mu1} bounds on $\johnftdinvvector_1$:
\begin{align*}
\johnweights_{y, 1}^{-1} \johnftdinvvector_1 \parenth{1- \johnftdinvvector_1 + \alpha \frac{\levjohn_{y, 1}}{\johnweights_{y, 1}} \johnftdinvvector_1 } &\leq \johnweights_{y, 1}^{-1} \frac{\johnweights_{y, 1}}{\johnweights_{y, 1} - \alpha \levjohn_{y, 1}} \parenth{1 - \parenth{1 - \alpha\frac{\levjohn_{y, 1}}{\johnweights_{y, 1}}} \frac{\johnweights_{y, 1}}{\johnweights_{y, 1} - \alpha \levjohn_{y, 1} + \alpha \levjohn_{y, 1}^2 }} \\
& = \frac{\alpha \levjohn_{y, 1}^2}{\parenth{\johnweights_{y, 1} - \alpha \levjohn_{y, 1}}\parenth{\johnweights_{y, 1} - \alpha \levjohn_{y, 1} + \alpha \levjohn_{y, 1}^2}} \\
& \leq \johnkappa^2,
\end{align*}
where in the last step we have used the facts that $\johnweights_{y, 1} \geq \levjohn_{y, 1}$ and $(1-\alpha)^{-1} = \johnkappa$.
Putting the pieces together, we obtain $\sum_{j=2}^\obs \johnftdinvvector_j^2 \johnweights_{y, j}^{-1} \leq \johnkappa^3,$
which is equivalent to our claim~\eqref{eq:john_mu_sum_of_terms_bound} for $i=1$.
% The same proof works for any other row $i \neq 1$. We conclude that
% \begin{align*}
%       \forall i \in [\obs]^2, 0 \leq \johnftdinvmatrix_{y, i, i} \leq \johnkappa \text{ and } \sum_{k \neq i} \johnftdinvmatrix_{y, i, k}^2 \johnweights_{k}^{-1} \leq \johnkappa^3.
% \end{align*}

It remains to prove our earlier claim~\eqref{eq:john_lower_bound_mu1}.
Writing equation~\eqref{eq:john_F_to_D_infinity_bound} separately for the first coordinate and for the rest of the coordinates, we obtain
\begin{subequations}
\begin{align}
  1 &= \parenth{1 - \alpha \levjohn_{y, 1} \johnweights_{y, 1}^{-1} + \alpha \levjohn_{y, 1, 1}^2 \johnweights_{y, j}^{-1}} \johnftdinvvector_1 + \alpha \sum_{j = 2}^\obs \levjohn_{y, 1, j}^2 \johnweights_{y, j}^{-1} \johnftdinvvector_j \label{eq:john_F_to_D_infinity_bound_dev1}, \quad \text{and} \\
  0 &= \parenth{\Ind_{\obs-1} - \alpha \johnlevmatrix_y' \johnweightmatrix_y'^{-1}} \begin{pmatrix}\johnftdinvvector_2 \\ \vdots \\ \johnftdinvvector_\obs \end{pmatrix} + \alpha \johnprojmatrix_y'^{(2)} \johnweightmatrix_y'^{-1}\begin{pmatrix}\johnftdinvvector_2 \\ \vdots \\ \johnftdinvvector_\obs \end{pmatrix} + \alpha \johnweights_{y, 1}^{-1} \johnftdinvvector_1 \begin{pmatrix} \levjohn_{y, 1, 2}^2 \\ \vdots \\ \levjohn_{y, 1, \obs}^2
\end{pmatrix}, \label{eq:john_F_to_D_infinity_bound_dev2}
\end{align}
\end{subequations}
where $\johnweightmatrix_y'$ (respectively $\johnlevmatrix_y', \johnprojmatrix_y'^{(2)}$) denotes the principal minor of $\johnweightmatrix_y$ (respectively $\johnlevmatrix_y, \johnprojmatrix_y^{(2)}$) obtained by excluding the first column and the first row.
Multiplying both sides of the equation~\eqref{eq:john_F_to_D_infinity_bound_dev2} from the left by $\begin{pmatrix}\johnftdinvvector_2, \cdots, \johnftdinvvector_\obs\end{pmatrix} \johnweightmatrix_y'^{-1}$, we obtain
\begin{align}
  0 = \sum_{j=2}^\obs \underbrace{\frac{1}{\johnweights_{y, j}}\parenth{1- \frac{\alpha\levjohn_{y, j}}{\johnweights_{y, j}}} \johnftdinvvector_{j}^2}_{c_{y, j}}
  + \alpha \underbrace{\begin{pmatrix}\johnftdinvvector_2, \cdots, \johnftdinvvector_\obs\end{pmatrix} \johnweightmatrix_y'^{-1} \johnprojmatrix_y'^{(2)} \johnweightmatrix_y'^{-1}\begin{pmatrix}\johnftdinvvector_2 \\ \vdots \\ \johnftdinvvector_\obs \end{pmatrix}}_{C_{y. 2}}
  + \alpha \frac{\johnftdinvvector_1}{\johnweights_{y, 1}} \sum_{j=2}^\obs \frac{\levjohn_{y, j}^2}{\johnweights_{y, j}} \johnftdinvvector_j.
  \label{eq:john_second_sum_mu}
\end{align}
Observing that $\alpha \in [0, 1]$ and $\johnweights_{y, j} \geq \levjohn_{y, j}$ for all $y \in \intP$ and $j \in [\obs]$, we obtain $c_{y, j} \geq 0$.
Further, note that $\johnweightmatrix_y'^{-1} \johnprojmatrix_y'^{(2)} \johnweightmatrix_y'^{-1}$ is a PSD matrix and hence we have that $C_{y, 2} \geq 0$.
Putting the pieces together, we have
\begin{align*}
  \alpha \frac{\johnftdinvvector_1}{\johnweights_{y, 1}} \sum_{j=2}^\obs \frac{\levjohn_{y, j}^2}{\johnweights_{y, j}} \johnftdinvvector_j \leq 0.
\end{align*}
Combining this inequality with equation~\eqref{eq:john_F_to_D_infinity_bound_dev1} yields the claim.
% \end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proof of Corollary~\ref{corollary:f_to_d_l1}} % (fold)
\label{sub:proof_of_corollary_corollary:f_to_d_l1}
% \begin{proof}[Proof of Corollary~\ref{corollary:f_to_d_l1}]
Without loss of generality, we can prove the result for $i=1$.
Applying Cauchy-Schwarz inequality, we have
\begin{align*}
\vecnorm{\johnftdinvvector}{1} &= \johnftdinvvector_1 + \sum_{j=2}^\obs \abss{\johnftdinvvector_j}
\leq \johnftdinvvector_1 + \sqrt{\sum_{j=2}^\obs \frac{\johnftdinvvector_j^2}{\johnweights_{y, j}} \cdot \sum_{j=2}^\obs \johnweights_{y, j}}
\leq \johnkappa +  \johnkappa^{3/2} \cdot \sqrt{1.5\ \dims}
\leq 3\sqrt{\dims} \johnkappa^{3/2},
\end{align*}
where to assert the last inequality we have used Lemma~\ref{lemma:f_to_d_matrix} and Lemma~\ref{lemma:john_first_bounds}\ref{item:john_weight_sum}.
The claim~\eqref{eq:john_mu_1_bound} follows.
Further, noting that the infinity norm of a matrix is the $\ell_1$-norm of its transpose, we obtain $\matsnorm{\parenth{\johnweightmatrix_y-\alpha\johnlaplacian_y}^{-1} \johnweightmatrix_y}{\infty} \leq 3 \sqrt{\dims} \johnkappa^{3/2}$ as claimed.
% \end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Proof of Lemmas from Section~\ref{sub:tail_bounds}} % (fold)
\label{sec:proof_of_lemmas_from_section_sub:tail_bounds}

In this section, we collect proofs of auxiliary lemmas from Section~\ref{sub:tail_bounds}.


\subsection{Proof of Lemma~\ref{lemma:john_whp_slackness}} % (fold)
\label{sub:proof_of_lemma_whp:slackness}

Using Lemma~\ref{lemma:john_closeness_of_slackness}, and the relation~\eqref{eq:john_z_x_relation} we have
\begin{align}
  \parenth{1 - \frac{\slack_{z, i}}{\slack_{x, i}}}^2  \leq 4\frac{r^2}{\johnkappa^4\dims^{3/2}} \rvg\tp\rvg,
  \label{eq:john_gaussian_bound_on_slackness}
\end{align}
where $\rvg\sim\NORMAL(0, \Ind_\dims)$.
Define
\begin{align}
  \Delta_\slack \defn \max_{i \in [\obs],\  v \in \overline{xz}}\left\vert 1 - \frac{\slack_{v, i}}{\slack_{x, i}}\right\vert.
  \label{eq:john_delta_s}
\end{align}
Using the standard Gaussian tail bound, we observe that $\Prob_{\rvg \sim \NORMAL(0, \Ind_n)} \brackets{\rvg \tp \rvg \geq \dims (1+\delta)} \leq 1 - \epsilon/4$ for $\delta  = \sqrt{\frac{2}{\dims}}$.
Plugging this bound in the inequality~\eqref{eq:john_gaussian_bound_on_slackness} and noting that for all $v \in \overline{xz}$ we have $\vecnorm{v-x}{\john_x} \leq \vecnorm{z-x}{\john_x} $, we obtain that
\begin{align*}
  \Prob_{z\sim \proposal_x}\brackets{\Delta_\slack  \leq \frac{2r^2 (1+\sqrt{2/\dims}\log(4/\epsilon)}{\johnkappa^4\sqrt{\dims}}} \geq 1 - \epsilon/4.
\end{align*}
Setting
\begin{align}
  \label{eq:john_whp_slackness_r_condition}
  r \leq 1/(25\sqrt{1+\sqrt{2}\log(4/\epsilon)}),
\end{align}
and noting that $\johnkappa^4\sqrt{\dims} \geq 1$ implies the claim~\eqref{eq:john_slack_whp}.
Hence, we obtain that $\Delta_\slack < .005/\johnkappa^2$  and consequently $\max_{i \in [\obs], v\in \overline{xz}} \slack_{x, i}/\slack_{v, i} \in (0.99, 1.01) $ with probability at least $1-\epsilon/4$.

We now claim that
\begin{align*}
  \max_{i \in [\obs], v \in \overline{xz}} \frac{\johnweights_{x, i}}{\johnweights_{v, i}} \in \brackets{1-24\johnkappa^2\Delta_\slack, 1+24\johnkappa^2\Delta_\slack}, \quad \text{ if } \Delta_\slack \leq \frac{1}{32\johnkappa^2}.
\end{align*}
The result follows immediately from this claim.
To prove the claim, note that equation~\eqref{eq:john_bound_on_ratio_of_johnweights} implies that if $\Delta_\slack  \leq \frac{1}{32\johnkappa^2}$, then
\begin{align*}
  \frac{\johnweights_{v, i}}{\johnweights_{x, i}} \in (e^{-8\johnkappa^2\Delta_\slack}, e^{8\johnkappa^2\Delta_\slack}) \quad \text{for all } i \in [\obs] \text{ and } v \in \overline{xz},
\end{align*}
which implies that
\begin{align*}
  \max_{i \in [\obs], v \in \overline{xz}} \frac{\johnweights_{x, i}}{\johnweights_{v, i}} \in (e^{-8\johnkappa^2\Delta_\slack}, e^{8\johnkappa^2\Delta_\slack}).
\end{align*}
Asserting the facts that $e^x \leq 1+3x $ and $e^{-x} \geq 1-3x$, for all $x \in [0, 1]$ yields the claim.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Proof of Lemma~\ref{lemma:john_gaussian_moment_bounds}} % (fold)
\label{sub:proof_of_lemma_lemma:john_gaussian_moment_bounds}

The proof once again makes use of the classical tail bounds for
polynomials in Gaussian random variables.
We restate the classical result stated in equation~\eqref{EqnJansonBound} for convenience.
For any $\dims \geq 1$,
any polynomial $P:\realdim \rightarrow \real$ of degree $\degree$, and
any $t \geq (2e)^{{\degree}/{2}}$, we have
\begin{align}
  \label{EqnJansonBound}
    \Prob\brackets{\abss{P(\rvg)} \geq t
      \parenth{\Exs{P(\rvg)}^2}^{\frac{1}{2}}} \leq \exp\parenth{-
      \frac{\degree}{2e} t^{{2}/{\degree}}},
\end{align}
where $\rvg \sim \NORMAL(0, \Ind_n)$ denotes a standard Gaussian vector in $n$ dimensions.

Recall the notation from equation~\eqref{eq:john_hat_a_hat_b} and observe that
% \begin{align*}
%   \hat{a}_{x, i} = \frac{\john_x^{-1/2} a_i}{s_{x, i}^2} \text{ and } \hat{b}_{x, i} = \john_x^{-1/2}A_x\Lambda_x \parenth{G_x - \alpha \Lambda_x}^{-1} e_i.
% \end{align*}
% We have
\begin{align}
  \vecnorm{\hat a_{x, i}}{2}^2 = \johnlocalslack_{x, i},
  \quad \text{and} \quad
  \hat a_{x, i}\tp \hat a_{x, j} = \johnlocalslack_{x, i, j}.
  \label{eq:john_hat_a_norm}
\end{align}
We also have
\begin{align}
  \sum_{i=1}^\obs \johnweights_{x, i} \hat a_{x, i} \hat a_{x, i}\tp =
  \john_x^{-1/2} \sum_{i=1}^\obs \johnweights_{x, i} \frac{ a_ia_i\tp}{s_{x, i}^2} \john_x^{-1/2}
  = \Ind_\dims.
  \label{eq:john_hat_a_a_Identity}
\end{align}
Further, using Lemma~\ref{lemma:f_to_d_l2} we obtain
\begin{align}
\sum_{i=1}^\obs \johnweights_{x, i} \hat{b}_{x, i}\hat{b}_{x, i} \tp
% &= \john_x^{-1/2}A_x\johnlaplacian_x \parenth{\johnweightmatrix_x - \alpha \johnlaplacian_x}^{-1} \parenth{\sum_{i=1}^\obs \johnweights_{x, i} e_i e_i \tp} \parenth{\johnweightmatrix_x - \alpha \johnlaplacian_x}^{-1} \johnlaplacian_x A_x\tp  \john_x^{-1/2} \notag \\
= \john_x^{-1/2}A_x\johnlaplacian_x \parenth{\johnweightmatrix_x - \alpha \johnlaplacian_x}^{-1} \johnweightmatrix_x \parenth{\johnweightmatrix_x - \alpha \johnlaplacian_x}^{-1} \johnlaplacian_x A_x\tp  \john_x^{-1/2}
% & \leq 4 \johnkappa^2 \john_x^{-1/2} \john_x \john_x^{-1/2} \notag \\
= 4 \johnkappa^2 \Ind_\dims.
\label{eq:john_john_hat_b_hat_b_Ind}
\end{align}
Throughout this section, we consider a fixed point $x \in \intP$.
For brevity in our notation, we drop the dependence on $x$ for terms like $\johnweights_{x, i}, \johnlocalslack_{x, i}, \hat a_{x, i}$ (etc.) and  denote them simply by $\johnweights_i, \johnlocalslack_i, \hat a_i$ respectively.

We introduce some matrices and vectors that would come in handy for our proofs.
\begin{align}
  B = \begin{bmatrix}
    \sqrt{\johnweights_1}\hat a_1\tp\\
    \vdots\\
    \sqrt{\johnweights_\obs}\hat a_\obs\tp
  \end{bmatrix},
  \quad
  B_b = \begin{bmatrix}
    \sqrt{\johnweights_1}\hat b_1\tp\\
    \vdots\\
    \sqrt{\johnweights_\obs}\hat b_\obs\tp
  \end{bmatrix},
  \quad
  v = \begin{bmatrix}
    \sqrt{\johnweights_1} \vecnorm{\hat a_1}{2}^2\\
    \vdots\\
    \sqrt{\johnweights_\obs} \vecnorm{\hat a_\obs}{2}^2
  \end{bmatrix},
  \quad\text{and}\quad
  v^{ab} = \begin{bmatrix}
    \sqrt{\johnweights_1} \hat a_1\tp\hat b_1\\
    \vdots\\
    \sqrt{\johnweights_\obs} \hat a_\obs\tp\hat b_\obs
  \end{bmatrix}.
\end{align}
We claim that
\begin{subequations}
  \begin{align}
    BB\tp \preceq \Ind_\obs, \quad\text{and}\quad
    B_bB_b\tp \preceq 4\johnkappa^2\Ind_\obs \label{eq:john_BB_and_BbBb}.
  \end{align}
To see these claims, note that equation~\eqref{eq:john_hat_a_a_Identity}
implies that $B\tp B = \Ind_\dims$ and consequently, $BB\tp$ is an orthogonal
projection matrix and $BB\tp \preceq \Ind_\obs$.
Next, note that from equation~\eqref{eq:john_john_hat_b_hat_b_Ind}
we have that $B_b\tp B_b \preceq \johnkappa^2\Ind_\dims$, which implies that
$B_b B_b\tp \preceq \johnkappa^2\Ind_\obs$.
In asserting both these arguments, we have used the fact that for any matrix $B$,
the matrices $BB\tp$ and $B\tp B$ are PSD and have same set of eigenvalues.

Next, we bound the $\ell_2$ norm of the vectors $v$ and $v^{ab}$:
\begin{align}
  \vecnorm{v}{2}^2 &= \sum_{i=1}^\obs \johnweights_i \johnlocalslack_i^2 \ \stackrel{\mathrm{Lem.}~\ref{ppt:john_all_properties}~\ref{item:john_theta_square_sigma_sum_bound}}{\leq} \ 4\dims, \quad \text{and} \label{eq:john_v2}\\
    % \vecnorm{v^{ab}}{2}^2 \leq 16 \johnkappa^2\dims.\label{eq:john_vab}
    \vecnorm{v^{ab}}{2}^2 &= \sum_{i=1}^\obs \johnweights_i \parenth{\hat{a}_i\tp\hat{b}_i}^2 \leq \sum_{i=1}^\obs \johnweights_i \vecnorm{\hat{a}_i}{2}^2 \vecnorm{\hat{b}_i}{2}^2 \leq 4 \sum_{i=1}^\obs \johnweights_i \vecnorm{\hat{b}_i}{2}^2
    = 4\trace(B_b\tp B_b)
    \stackrel{\mathrm{eqn.}~\eqref{eq:john_BB_and_BbBb}}{\leq} 16 \johnkappa^2 \dims.\label{eq:john_vab}
\end{align}
\end{subequations}
We now prove the five claims of the lemma separately.
% Using equation~\eqref{eq:john_hat_a_norm} and Lemma~\ref{lemma:john_first_bounds}~\ref{item:john_theta_bound}, we find that
% \begin{align*}
%     \vecnorm{v}{2}^2 = \sum_{i=1}^\obs \johnweights_i \johnlocalslack_i^2 \leq 4\dims,
% \end{align*}
% which implies claim~\eqref{eq:john_v2}.
% To bound the $\ell_2$-norm of the vector $v^{ab}$, observe that
% \begin{align}
%   \sum_{i=1}^\obs \johnweights_i \vecnorm{\hat{b}_i}{2}^2 = \trace(B_b\tp B_b) \in[0, 4\johnkappa^2\dims]
%   \label{eq:john_sum_of_bi}
% \end{align}
% and consequently
% \begin{align*}
% \vecnorm{v^{ab}}{2}^2 = \sum_{i=1}^\obs \johnweights_i \parenth{\hat{a}_i\tp\hat{b}_i}^2 \leq \sum_{i=1}^\obs \johnweights_i \vecnorm{\hat{a}_i}{2}^2 \vecnorm{\hat{b}_i}{2}^2 \leq 4 \sum_{i=1}^\obs \johnweights_i \vecnorm{\hat{b}_i}{2}^2 \leq 16 \johnkappa^2 \dims.
%  \end{align*}



\subsubsection{Proof of bound~(\ref{eq:john_john_quadratic})}
\label{ssub:proof_of_part_item:john_quadratic}
Using Isserlis’ theorem~\citep{isserlis1918formula} for fourth order Gaussian moments, we have
\begin{align*}
  \Exs \parenth{\sum_{i=1}^\obs \johnweights_i \parenth{\hat{a}_i\tp \rvg}^2}^2
  % &=
  % \sum_{i,j=1}^\obs \johnweights_i \johnweights_j \Exs
  % \parenth{\hat{a}_i\tp \rvg}^2 \parenth{\hat{a}_j\tp \rvg}^2 \\
%
 = \sum_{i,j=1}^\obs \johnweights_i \johnweights_j \parenth{
    \vecnorm{\hat{a}_i}{2}^2\vecnorm{\hat{a}_j}{2}^2 + 2
    \parenth{\hat{a}_i\tp \hat{a}_j}^2 }
%
 = \sum_{i,j=1}^\obs \johnweights_i \johnweights_j
  \parenth{\johnlocalslack_{i}\johnlocalslack_{j} + 2
    \johnlocalslack_{i, j}^2 }
%
% & \stackrel{(i)}{=} 16 \dims^2 + 8 \dims \\
& \leq 24 \dims^2,
\end{align*}
where the last follows from Lemma~\ref{ppt:john_all_properties}. Applying the bound~\eqref{EqnJansonBound} with $k=2$ and $t = e \log(\frac{16}{\epsilon})$. Note that the bound is valid since $t \geq (2e)$ for all $\epsilon \in (0, \johnepsilonconst]$.

\subsubsection{Proof of bound~(\ref{eq:john_john_cubic})}
\label{ssub:proof_of_part_item:john_cubic}
Applying Isserlis’ theorem for Gaussian moments, we obtain
\begin{align*}
\Exs \parenth{\sum_{i=1}^\obs \johnweights_i \parenth{\hat{a}_i \tp \xi}^3}^2 = 9\underbrace{\sum_{i,j=1}^\obs \johnweights_i \johnweights_j \vecnorm{\hat{a}_i}{2}^2 \vecnorm{\hat{a}_j}{2}^2 \parenth{\hat{a}_i\tp \hat{a}_j}}_{=:N_1} + 6 \underbrace{\sum_{i,j=1}^\obs \johnweights_i \johnweights_j \parenth{\hat{a}_i\tp \hat{a}_j}^3}_{=:N_2}.
\end{align*}
We claim that $N_1 \leq 4\dims$ and $N_2 \leq 4\dims$.
Assuming these claims as given at the moment, we now complete the proof.
We have $\Exs \parenth{\sum_{i=1}^\obs \johnweights_i \parenth{\hat{a}_i \tp \xi}^3}^2 \leq 60 \dims$.
Applying the bound~\eqref{EqnJansonBound} with $\degree = 3$ and $t =
\parenth{\frac{2e}{3} \log \parenth{\frac{16}{\epsilon}}}^{3/2}$, and verifying that $t \geq \parenth{2e}^{3/2}$ for $\epsilon \in (0, \johnepsilonconst]$ yields the claim.


We now turn to prove the bounds on $N_1$ and $N_2$.
We have
\begin{align*}
  N_1 = \sum_{i,j=1}^\obs \johnweights_i {\vecnorm{\hat{a}_i}{2}^2 \hat{a}_i\tp
    \johnweights_j
    \vecnorm{\hat{a}_j}{2}^2 \hat{a}_j} &= \vecnorm{\sum_{i=1}^\obs
     \johnweights_i \vecnorm{\hat{a}_i}{2}^2 \hat{a}_i }{2}^2
  = \vecnorm{B\tp v}{2}^2
  \stackrel{\mathrm{eqn.}~\eqref{eq:john_BB_and_BbBb}}{\leq} \vecnorm{v}{2}^2
  \stackrel{\mathrm{eqn.}~\eqref{eq:john_v2}}{\leq} 4\dims.
\end{align*}
Next, applying Cauchy-Schwarz inequality and using equation~\eqref{eq:john_hat_a_norm}, we obtain
\begin{align*}
  N_2 = \sum_{i,j=1}^\obs \johnweights_i \johnweights_j
  \parenth{\hat{a}_i\tp \hat{a}_j}^3
  % &\stackrel{\mathmakebox[\widthof{=======}]{ (\mathrm{C-S})
  % }}{\leq} \sum_{i,j=1}^\obs \johnweights_i \johnweights_j
  % \parenth{\hat{a}_i\tp \hat{a}_j}^2
  % \vecnorm{\hat{a}_i}{2}\vecnorm{\hat{a}_j}{2} \\
%
& \leq \sum_{i,j=1}^\obs \johnweights_i \johnweights_j
  \johnlocalslack_{i, j}^2 \sqrt{\johnlocalslack_i\johnlocalslack_j}
%
& \stackrel{\mathmakebox[\widthof{====}]{
      (\mathrm{Lem.}~\ref{lemma:john_first_bounds}~\ref{item:john_theta_bound})
  }}{\leq} 4 \sum_{i,j=1}^\obs
  \johnweights_i \johnweights_j \johnlocalslack_{i, j}^2
& \stackrel{\mathmakebox[\widthof{=====}]{
      (\mathrm{Lem.}~\ref{ppt:john_all_properties}~\ref{item:john_theta_properties})
  }}{\leq} 4 \sum_{i=1}^\obs
  \johnweights_i \johnlocalslack_i
& = 4\dims.
\end{align*}


% \paragraph{Bounding $N_1$:}
% \label{par:john_bounding_n1}
% We have
% \begin{align*}
%   \sum_{i,j=1}^\obs \johnweights_i {\vecnorm{\hat{a}_i}{2}^2 \hat{a}_i\tp
%     \johnweights_j
%     \vecnorm{\hat{a}_j}{2}^2 \hat{a}_j} &= \vecnorm{\sum_{i=1}^\obs
%      \johnweights_i \vecnorm{\hat{a}_i}{2}^2 \hat{a}_i }{2}^2
%   = \vecnorm{B\tp v}{2}^2
%   \stackrel{\mathrm{eqn.}~\eqref{eq:john_BB_and_BbBb}}{\leq} \vecnorm{v}{2}^2
%   \stackrel{\mathrm{eqn.}~\eqref{eq:john_v2}}{\leq} 4\dims.
% \end{align*}
% where inequality $(i)$ follows from equation~\eqref{eq:john_BB_and_BbBb}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \paragraph{Bounding $N_2$:}
% \label{par:john_bounding_n2}
% We have that
% \begin{align*}
%   \sum_{i,j=1}^\obs \johnweights_i \johnweights_j
%   \parenth{\hat{a}_i\tp \hat{a}_j}^3
%   &\stackrel{\mathmakebox[\widthof{=======}]{ (\mathrm{C-S})
%   }}{\leq} \sum_{i,j=1}^\obs \johnweights_i \johnweights_j
%   \parenth{\hat{a}_i\tp \hat{a}_j}^2
%   \vecnorm{\hat{a}_i}{2}\vecnorm{\hat{a}_j}{2} \\
% %
% & \stackrel{\mathmakebox[\widthof{=======}]{
%       (\mathrm{eqn.}~\ref{eq:john_hat_a_norm})
%   }}{\leq} \sum_{i,j=1}^\obs \johnweights_i \johnweights_j
%   \johnlocalslack_{i, j}^2 \sqrt{\johnlocalslack_i\johnlocalslack_j} \\
% %
% & \stackrel{\mathmakebox[\widthof{=======}]{
%       (\mathrm{Lem.}~\ref{lemma:john_first_bounds}~\ref{item:john_theta_bound})
%   }}{\leq} 4 \sum_{i,j=1}^\obs
%   \johnweights_i \johnweights_j \johnlocalslack_{i, j}^2 \\
% & \stackrel{\mathmakebox[\widthof{=======}]{
%       (\mathrm{Lem.}~\ref{ppt:john_all_properties}~\ref{item:john_theta_properties})
%   }}{\leq} 4 \sum_{i}^\obs
%   \johnweights_i \johnlocalslack_i\\
% & \mathmakebox[\widthof{=======}]{=} 4n.
% \end{align*}


\subsubsection{Proof of bound~(\ref{eq:john_john_cubic_f})}
\label{ssub:proof_of_part_item:john_cubic_f}

Using Isserlis’ theorem for Gaussian moments, we have
\begin{multline*}
\Exs \parenth{\sum_{i=1}^\obs \johnweights_i \parenth{\hat{a}_i \tp \xi}^2 \parenth{\hat{b}_{x,i} \tp \xi}}^2
= \underbrace{\sum_{i, j=1}^\obs \johnweights_i \johnweights_j \vecnorm{\hat{a}_i}{2}^2 \vecnorm{\hat{a}_j}{2}^2 \parenth{\hat{b}_i\tp \hat{b}_j}}_{:=N_3}
+ 4 \underbrace{\sum_{i, j=1}^\obs \johnweights_i \johnweights_j \parenth{\hat{a}_i \tp \hat{a}_j} \parenth{\hat{a}_i \tp \hat{b}_i}  \parenth{\hat{a}_j\tp \hat{b}_j}}_{:=N_4} \\
+ 4 \underbrace{\sum_{i, j=1}^\obs \johnweights_i \johnweights_j \vecnorm{\hat{a}_i}{2}^2 \parenth{\hat{b}_i\tp \hat{a}_j} \parenth{\hat{a}_j\tp \hat{b}_j}}_{:=N_5}
+ 2 \underbrace{\sum_{i, j=1}^\obs \johnweights_i \johnweights_j \parenth{\hat{a}_i \tp \hat{a}_j}^2 \parenth{\hat{b}_i\tp \hat{b}_j}}_{:=N_6}
+ 4 \underbrace{\sum_{i, j=1}^\obs \johnweights_i \johnweights_j \parenth{\hat{a}_i \tp \hat{a}_j} \parenth{\hat{a}_i \tp \hat{b}_j} \parenth{\hat{b}_i\tp \hat{a}_j}}_{:=N_7}
\end{multline*}
% \begin{align*}
% \Exs \parenth{\sum_{i=1}^\obs \johnweights_i \parenth{\hat{a}_i \tp \xi}^2 \parenth{\hat{b}_{x,i} \tp \xi}}^2
% &= \underbrace{\sum_{i, j=1}^\obs \johnweights_i \johnweights_j \vecnorm{\hat{a}_i}{2}^2 \vecnorm{\hat{a}_j}{2}^2 \parenth{\hat{b}_i\tp \hat{b}_j}}_{:=N_3} \\
% &+ 4 \underbrace{\sum_{i, j=1}^\obs \johnweights_i \johnweights_j \parenth{\hat{a}_i \tp \hat{a}_j} \parenth{\hat{a}_i \tp \hat{b}_i}  \parenth{\hat{a}_j\tp \hat{b}_j}}_{:=N_4} \\
% &+ 4 \underbrace{\sum_{i, j=1}^\obs \johnweights_i \johnweights_j \vecnorm{\hat{a}_i}{2}^2 \parenth{\hat{b}_i\tp \hat{a}_j} \parenth{\hat{a}_j\tp \hat{b}_j}}_{:=N_5} \\
% &+ 2 \underbrace{\sum_{i, j=1}^\obs \johnweights_i \johnweights_j \parenth{\hat{a}_i \tp \hat{a}_j}^2 \parenth{\hat{b}_i\tp \hat{b}_j}}_{:=N_6} \\
% &+ 4 \underbrace{\sum_{i, j=1}^\obs \johnweights_i \johnweights_j \parenth{\hat{a}_i \tp \hat{a}_j} \parenth{\hat{a}_i \tp \hat{b}_j} \parenth{\hat{b}_i\tp \hat{a}_j}}_{:=N_7}
% \end{align*}
% \yccomment{The first three terms have only one $i,j$ cross term, while the last two terms have three. Like in previous proof, the first three terms use the projection idea. While the last two terms uses Cauchy-Schwarz to bound directly. }
We claim that all terms $N_k \leq 16\johnkappa^2 \dims, k \in \braces{3, 4, 5, 6, 7}$.
Putting the pieces together, we have
\begin{align*}
\Exs \parenth{\sum_{i=1}^\obs \johnweights_i \parenth{\hat{a}_i \tp \xi}^2 \parenth{\hat{b}_{x,i} \tp \xi}}^2 \leq 240 \johnkappa^2 \dims.
\end{align*}
Applying the bound~\eqref{EqnJansonBound} with $\degree = 3$ and $t =
\parenth{\frac{2e}{3} \log \parenth{\frac{16}{\epsilon}}}^{3/2}$ yields the claim. Note that for the given definition of $t$, we have $t \geq \parenth{2e}^{3/2}$ for $\epsilon \in (0, \johnepsilonconst]$ so that the bound~\eqref{EqnJansonBound} is valid.

% It is now left to prove the bounds on $N_k$ for $k \in \braces{3, 4, 5, 6, 7}$.
% \paragraph{Bounding $N_3$:}
% \label{par:john_bounding_n3}
% Observe that
% \begin{align*}
%   \sum_{i,j=1}^\obs \johnweights_i {\vecnorm{\hat{a}_i}{2}^2 \hat{b}_i\tp
%     \johnweights_j
%     \vecnorm{\hat{a}_j}{2}^2 \hat{b}_j} &= \vecnorm{\sum_{i=1}^\obs
%      \johnweights_i \vecnorm{\hat{a}_i}{2}^2 \hat{b}_i }{2}^2
%   = \vecnorm{B_b \tp v}{2}^2
%   \stackrel{(i)}{\leq} 4 \johnkappa^2 \vecnorm{v}{2}^2,
%   \stackrel{(ii)}{\leq} 16 \johnkappa^2 \dims
% \end{align*}
% where step $(i)$ follows from equation~\eqref{eq:john_BB_and_BbBb} and step (ii) from equation~\eqref{eq:john_v2}.

% \paragraph{Bounding $N_4$:}
% \label{par:john_bounding_n4}
% Using equation~\eqref{eq:john_BB_and_BbBb} and \eqref{eq:john_vab}, we find that
% \begin{align*}
% \sum_{i, j=1}^\obs \johnweights_i \johnweights_j \parenth{\hat{a}_i \tp \hat{a}_j} \parenth{\hat{a}_i \tp \hat{b}_i}  \parenth{\hat{a}_j\tp \hat{b}_j} = \vecnorm{B \tp v^{ab}}{2}^2 \leq \vecnorm{v^{ab}}{2}^2
% \leq 16\johnkappa^2\dims.
% \end{align*}

% \paragraph{Bounding $N_5$:}
% \label{par:john_bounding_n5}
% Applying Cauchy-Schwarz inequality, we obtain
% \begin{align*}
% \sum_{i, j=1}^\obs \johnweights_i \johnweights_j \vecnorm{\hat{a}_i}{2}^2 \parenth{\hat{b}_i\tp \hat{a}_j} \parenth{\hat{a}_j\tp \hat{b}_j} = \parenth{B\tp v^{ab}}\tp \parenth{B_b \tp v} \leq \vecnorm{B \tp v^{ab}}{2} \vecnorm{B_b \tp v}{2} \leq 16 \johnkappa^2 \dims,
% \end{align*}
% where in the last step we have used the bounds on $\ell_2$-norms of the vectors $B \tp v^{ab}$ and $B_b\tp v$ from the previous parts.

% \paragraph{Bounding $N_6$:}
% \label{par:john_bounding_n6}
% Using Cauchy-Schwarz inequality, we have
% \begin{align*}
% \sum_{i, j=1}^\obs \johnweights_i \johnweights_j \parenth{\hat{a}_i \tp \hat{a}_j}^2 \parenth{\hat{b}_i\tp \hat{b}_j}
% & \leq \sum_{i, j=1}^\obs \johnweights_i \johnweights_j \parenth{\hat{a}_i \tp \hat{a}_j}^2 \parenth{\vecnorm{\hat{b}_i}{2}^2 +  \vecnorm{\hat{b}_j}{2}^2}/2\\
% & = \sum_{i, j=1}^\obs \johnweights_i \johnweights_j \parenth{\hat{a}_i \tp \hat{a}_j}^2 \vecnorm{\hat{b}_i}{2}^2\\
% & = \sum_{i}^\obs \johnweights_i \vecnorm{\hat{a}_i}{2}^2 \vecnorm{\hat{b}_i}{2}^2 \\
% & \leq 4 \sum_{i}^\obs \johnweights_i \vecnorm{\hat{b}_i}{2}^2\\
% & \leq 16 \johnkappa^2 \dims,
% \end{align*}
% where the last step follows from equation~\eqref{eq:john_sum_of_bi}.

% \paragraph{Bounding $N_7$:}
% \label{par:john_bounding_n7}
% Applying Lemma~\ref{lemma:john_first_bounds}~\ref{item:john_theta_bound} and using equation~\eqref{eq:john_sum_of_bi} we obtain
% \begin{align*}
% \sum_{i, j=1}^\obs \johnweights_i \johnweights_j \parenth{\hat{a}_i \tp \hat{a}_j} \parenth{\hat{a}_i \tp \hat{b}_j} \parenth{\hat{b}_i\tp \hat{a}_j}
% & \leq \sum_{i, j=1}^\obs \johnweights_i \johnweights_j \vecnorm{\hat{a}_i}{2}\vecnorm{\hat{a}_j}{2} \parenth{\parenth{\hat{a}_i \tp \hat{b}_j}^2 + \parenth{\hat{b}_i\tp \hat{a}_j}^2}/2 \\
% & \leq 4 \sum_{i, j=1}^\obs \johnweights_i \johnweights_j \parenth{\hat{a}_i \tp \hat{b}_j}^2 \\
% & = 4 \sum_{j=1}^\obs \johnweights_j \parenth{\hat{b}_j \tp \hat{b}_j} \\
% & \leq 16 \johnkappa^2 \dims.
% \end{align*}


It is now left to prove the bounds on $N_k$ for $k \in \braces{3, 4, 5, 6, 7}$.
We have
\begin{align*}
  N_3 &= \sum_{i,j=1}^\obs \johnweights_i {\vecnorm{\hat{a}_i}{2}^2 \hat{b}_i\tp
    \johnweights_j
    \vecnorm{\hat{a}_j}{2}^2 \hat{b}_j} = \vecnorm{\sum_{i=1}^\obs
     \johnweights_i \vecnorm{\hat{a}_i}{2}^2 \hat{b}_i }{2}^2
  = \vecnorm{B_b \tp v}{2}^2\
  \stackrel{\mathrm{eqn.}~\eqref{eq:john_BB_and_BbBb}}{\leq} 4 \johnkappa^2 \vecnorm{v}{2}^2\
 = \stackrel{\mathrm{eqn.}~\eqref{eq:john_v2}}{\leq} 16 \johnkappa^2 \dims,\\
 N_4 &= \sum_{i, j=1}^\obs \johnweights_i \johnweights_j \parenth{\hat{a}_i \tp \hat{a}_j} \parenth{\hat{a}_i \tp \hat{b}_i}  \parenth{\hat{a}_j\tp \hat{b}_j} = \vecnorm{B \tp v^{ab}}{2}^2\ \
 \stackrel{\mathrm{eqn.}~\eqref{eq:john_BB_and_BbBb}}{\leq} \vecnorm{v^{ab}}{2}^2\ \
\stackrel{\mathrm{eqn.}~\eqref{eq:john_vab}}{\leq} 16\johnkappa^2\dims, \quad \text{and}\\
N_5 &=\sum_{i, j=1}^\obs \johnweights_i \johnweights_j \vecnorm{\hat{a}_i}{2}^2 \parenth{\hat{b}_i\tp \hat{a}_j} \parenth{\hat{a}_j\tp \hat{b}_j} = \parenth{B\tp v^{ab}}\tp \parenth{B_b \tp v} \
\stackrel{\mathrm{C-S}}{\leq} \vecnorm{B \tp v^{ab}}{2} \vecnorm{B_b \tp v}{2} \ \leq 16 \johnkappa^2 \dims.
\end{align*}
For the term $N_6$, we have
\begin{align*}
N_6 = \sum_{i, j=1}^\obs \johnweights_i \johnweights_j \parenth{\hat{a}_i \tp \hat{a}_j}^2 \parenth{\hat{b}_i\tp \hat{b}_j}
& \stackrel{\mathmakebox[\widthof{=======}]{(\mathrm{C-S})}}{\leq}
\frac{1}{2}\sum_{i, j=1}^\obs \johnweights_i \johnweights_j \parenth{\hat{a}_i \tp \hat{a}_j}^2 \parenth{\vecnorm{\hat{b}_i}{2}^2 +  \vecnorm{\hat{b}_j}{2}^2}\\
& \stackrel{\mathmakebox[\widthof{=======}]{(\mathrm{symm. in}~i, j)}}{=} \sum_{i, j=1}^\obs \johnweights_i \johnweights_j \parenth{\hat{a}_i \tp \hat{a}_j}^2 \vecnorm{\hat{b}_i}{2}^2\\
& \stackrel{\mathmakebox[\widthof{=======}]{(\mathrm{eqn.}~\eqref{eq:john_hat_a_a_Identity})}}{\leq} \sum_{i=1}^\obs \johnweights_i \vecnorm{\hat{a}_i}{2}^2 \vecnorm{\hat{b}_i}{2}^2 \\
& \stackrel{\mathmakebox[\widthof{=======}]{(\mathrm{Lem.}~\ref{lemma:john_first_bounds}\ref{item:john_theta_bound})}}{\leq} 4 \sum_{i=1}^\obs \johnweights_i \vecnorm{\hat{b}_i}{2}^2\\
& \stackrel{\mathmakebox[\widthof{=======}]{(\mathrm{eqn.}~\eqref{eq:john_vab})}}{\leq} 16 \johnkappa^2 \dims.
\end{align*}
The bound on the term $N_7$ can be obtained in a similar fashion.
% \paragraph{Bounding $N_7$:}
% \label{par:john_bounding_n7}
% Applying Lemma~\ref{lemma:john_first_bounds}~\ref{item:john_theta_bound} and using equation~\eqref{eq:john_sum_of_bi} we obtain
% \begin{align*}
% N_7 = \sum_{i, j=1}^\obs \johnweights_i \johnweights_j \parenth{\hat{a}_i \tp \hat{a}_j} \parenth{\hat{a}_i \tp \hat{b}_j} \parenth{\hat{b}_i\tp \hat{a}_j}
% & \leq \frac{1}{2} \sum_{i, j=1}^\obs \johnweights_i \johnweights_j \vecnorm{\hat{a}_i}{2}\vecnorm{\hat{a}_j}{2} \parenth{\parenth{\hat{a}_i \tp \hat{b}_j}^2 + \parenth{\hat{b}_i\tp \hat{a}_j}^2} \\
% & \leq 4 \sum_{i, j=1}^\obs \johnweights_i \johnweights_j \parenth{\hat{a}_i \tp \hat{b}_j}^2 \\
% & = 4 \sum_{j=1}^\obs \johnweights_j \parenth{\hat{b}_j \tp \hat{b}_j} \\
% & \leq 16 \johnkappa^2 \dims.
% \end{align*}


\subsubsection{Proof of bound~(\ref{eq:john_john_fourth})}
\label{ssub:proof_of_part_item:john_fourth}

Observe that $\hat{a}_i\tp \rvg\sim \NORMAL\parenth{0,
  \johnlocalslack_i}$ and hence $\Exs\parenth{\hat{a}_i\tp
  \rvg}^8 = 105\, \johnlocalslack_i^4$.
  Thus, we have
\begin{align*}
\Exs \parenth{\sum_{i=1}^\obs \johnweights_i
  \parenth{\hat{a}_i\tp \rvg}^4}^2 &
\stackrel{{\mathrm{C-S}}}{\leq}
\sum_{i,j=1}^\obs \johnweights_i \johnweights_j
\parenth{\Exs\parenth{\hat{a}_i\tp \rvg}^8}^{\frac{1}{2}}
\parenth{\Exs\parenth{\hat{a}_j\tp \rvg}^8}^{\frac{1}{2}}
%
= 105 \sum_{i,j=1}^\obs
\johnweights_i \johnweights_j \johnlocalslack_i^2
\johnlocalslack_j^2
= 105 \parenth{\sum_{i=1}^\obs \johnweights_i \johnlocalslack_i^2}^2.
% \stackrel{\mathmakebox[\widthof{====}]{(\mathrm{Lem.}~\ref{ppt:john_all_properties})}} {\leq} 1680\, \dims^2 .
\end{align*}
Now applying Lemma~\ref{ppt:john_all_properties}, we obtain that $\Exs \parenth{\sum_{i=1}^\obs \johnweights_i \parenth{\hat{a}_i\tp \rvg}^4}^2 \leq 1680 \dims^2$.
Consequently, applying the bound~\eqref{EqnJansonBound} with $\degree = 4$ and $t =
\parenth{\frac{e}{2} \log \parenth{\frac{16}{\epsilon}}}^{2}$ and noting that $t \geq \parenth{2e}^{2}$ for $\epsilon \in (0, \johnepsilonconst]$, yields the claim.


\subsubsection{Proof of bound~(\ref{eq:john_john_sixth})}
\label{ssub:proof_of_part_item:john_sixth}
Using the fact that $\Exs\parenth{\hat{a}_i\tp
  \rvg}^{12} = 945\, \johnlocalslack_i^6$ and an argument similar to the previous part yields that $\Exs \parenth{\sum_{i=1}^\obs \johnweights_i
  \parenth{\hat{a}_i\tp \rvg}^6}^2 \leq 15120 \dims^2$.

Finally, applying the bound~\eqref{EqnJansonBound} with $\degree = 6$ and $t =
\parenth{\frac{e}{3} \log \parenth{\frac{16}{\epsilon}}}^{3}$, and verifying that $t \geq \parenth{2e}^{3}$ for $\epsilon \in (0, \johnepsilonconst]$, yields the claim.



